How generic is eternal inflation?

Everlasting inflation has far-reaching implications for cosmology and the standing of self-localizing inferences made by observers, which have been subjects of renewed interest in light of the growing acceptance of theory landscapes and the attendant anthropic arguments. Under what assumptions and to what extent does inflation generically produce an eternal "multiverse," without fine-tuning with respect to measures over the space of inflationary cosmologies driven by a single minimally coupled scalar field? We address this and related questions with numerical simulations of inflationary dynamics across populations of randomly generated inflation models, instantiating a few particular simply-defined measures.

==> Generic/candidate_measures.tex <==

\section{Candidate Measures}

Which considerations have passed muster in the literature, in informing proposed measures over cosmological models?
Are simpler measures always better?
In order to avoid the impression of being finely-tuned {\it ab initio}, the measure should not encode too much {\it a priori} knowledge about the kinds of universes it is to produce.
Here we briefly discuss three possible measures on the effective potential, initial conditions, or both; and 

\paragraph{No-Boundary}
The No-Boundary proposal presented in \cite{PhysRevD.28.2960} establishes criteria for spacetime to behave classically at late times -- a prerequisite for the project of interpreting early universe cosmology in terms of an inflationary epoch.
It attempts to assign a ``wave function of the Universe'' -- the No-Boundary Wave Function (NBWF) -- derived from simple arguments in such a way as to evade specification of past boundary conditions.
It yields a measure over the classical history of the inflaton given a pre-defined potential function.

The authors draw a distinction between {\it bottom-up} versus {\it top-down} probabilities -- those prescribed by quantum theory and the NBWF versus those further conditioned on conditions needed to reproduce observational data, respectively.
(We generally direct our attention to the top-down variety.)
%
The No-Boundary Measure \cite{noboundary} assigns higher weight to models with very few $e$-folds of inflation beyond the minimum required to solve the horizon problem.
Saddle points with sharp curvature are disfavored; broad saddle points can behave classically at late times.
To evade the preference for few $e$-folds, the authors advocate a volume weighting of $\exp(3\mathcal N_E)$ in their calculation of top-down probabilities -- after this adjustment, a large number of $e$-folds is slightly preferred in approximately quadratic models.  
The criterion for volume weighting to outpace suppression from the action in the NBWF is equivalent to that for stochastic eternal inflation to within a factor of order unity.
%\[ \Psi(b,\chi) \approx \exp \left[ - I_R(b,\chi) + i S(b,\chi) \right] \]
%
The No-Boundary Measure ties the presence or absence of eternal inflation in our past with the Gaussianity of scalar density perturbations.
%
%
%NBWF favors a small number of $e$-foldings, but volume weighting compensates.  What if no volume weighting?
%
%Justification for Measure A?
%``the most probable histories started in an unstable de Sitter like state near a broad saddle-point''

%Classicality constraint: minimum amount of scalar field energy at early times to behave classically at late times

\paragraph{Refined de Sitter Swampland}
The ``refined'' de Sitter Swampland Conjecture \cite{Garg:2018reu} relaxes the requirements of the original somewhat, by allowing either the first derivative constraint in \eqref{dSswamp} or a new second derivative constraint \eqref{refinedswamp} to satisfy the criterion.  We can take the constraints as specifying a rudimentary measure over potentials and initial conditions: the field is sampled from regions of a potential in which these conditions are satisfied, while potentials with any or more of such regions are favored by the measure.
This can be viewed as using the landscape itself as a measure, keeping only the basins of attraction for which completion to quantum gravity is attainable.

The de Sitter swampland measure is too general, and does not give a natural prescription for probabilities apart from whether a small number of constraints on the potential are valid.
It seems like an additional constraint to be administered to a broader measure, cutting away a large portion of parameter space.

\paragraph{QFT Plausibility/Complexity}

A possibility not discussed in the literature -- though the motivation is often recognized as a value -- is to weight effective potentials in terms of the complexity to reproduce them from allowed interaction terms in quantum field theory.
In this measure, a quadratic potential -- corresponding to a simple massive scalar field -- would have high weight; a Higgs-like potential with quadratic and quartic contributions would not be far behind.
Potentials with terms of a single field taken to a power greater than 4 are disallowed, etc.
Unnatural potential shapes with wiggles and scaling discrepancies from one interval of field space to another would be heavily penalized.

A QFT complexity measure would require many priors assigned to the various parameters characterizing each term in the Lagrangian, and a mixture of continuous (parameters) and discrete (terms present or not) outcome spaces.

\paragraph{Takeaways}

Each of the measures discussed above presents problems when it comes to sampling from the distribution to compute statistics of eternality and observables.  
How does one draw random samples from the No-Boundary Measure, for instance?
We are limited to the most general statements about the behavior of late-time classical configurations, of which quick work has been made in the literature.
%
%In \cite{Olum2012} it is argued that no measure that accounts for volume-weighting meets a set of reasonable axioms in a satisfactory way.}
%
We are in search of a measure that both prescribes well defined probabilities and can be easily sampled numerically; to accomplish this may mean to sacrifice on aesthetic qualities of realism or sophistication.


==> Generic/ch-hybrid-inflation.tex <==


% \section{Specific Constructions of Viable Non-Eternal Inflation}

\chapter{Case Study: Hybrid Inflation}
\label{sec:constructions}

\begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{Figures/hybridpotential}
    \caption[{Potential for Hybrid Inflation.}]{Potential for hybrid inflation.}
\end{figure}

%To exemplify our approach, we can look at specific constructuions of viable inflation (by many metrics, in any case) that are commonly understood not to be generically eternal.
%
Hybrid inflation is a class of models in which eternal inflation is demonstrated not to be generic with respect to choice of initial conditions given a uniform measure, for a broad range of parameters defining the potential.
We can use it as a template to exemplify our approach.
The model first introduced by Linde \cite{linde1994hybrid} and further expanded in .
% that produced inflation with coupling parameters of order one, eliminating the need for fine-tuning.  
features two coupled scalar fields, the inflaton $\phi$ and a Higgs-like timer field $\sigma$, governed by the potential
\begin{equation} V(\phi,\sigma) = \frac12{m^2} \phi^2 + \frac1{4\lambda} (M^2 - \lambda \sigma^2)^2 + \frac12{g^2} \phi^2 \sigma^2 \label{hybrid_potential} \end{equation}
% The effective mass of the $\sigma$ field is given by $M_\sigma^2(\phi) = g^2\phi^2 - M^2$.  
If $\phi$ starts out much larger than the critical value $\phi_c \equiv M/g$, the curvature in $\sigma$ given by $M_\sigma^2(\phi) = g^2\phi^2 - M^2$ is correspondingly large and positive, and the system quickly settles to the local minimum at $\sigma = 0$ -- the floor of the ``inflationary valley.''  
In this regime, the model behaves effectively as a single-field quadratic model with an additional constant positive vacuum energy.  
The potential \eqref{hybrid_potential} reduces to
\begin{equation} V(\phi,0) = \frac12 m^2 \phi^2 + \frac{M^4}{4\lambda} = \frac12 m^2 \left( \phi^2 + a^2 M_P^2 \right), \label{valley} \end{equation}
where $a^2 \equiv \widebar M^4/2\lambda \widebar m^2$ and $M_P \equiv (8\pi G)^{-1/2}$ is the reduced Planck mass.\footnote{We have introduced an overline notation indicating that the quantity 
% is expressed in natural units, with $M_P = 1$:
has been made dimensionless by adding or removing powers of $M_P$: 
$\widebar m \equiv m/M_P$, $\widebar \phi \equiv \phi/M_P$, $\widebar V \equiv V/M_P^4$, etc. The parameters $m$ and $M \gg m$ have dimensions of mass, and $g$ and $\lambda$ are dimensionless.}

Slow roll of the initially large inflaton field is interrupted by a phase transition at $\phi_c$, at which point $M_\sigma^2$ becomes negative.  
At that point, the system rapidly rolls down to one of the two global minima at $\phi=0,\;\sigma=\pm M/\sqrt{\lambda}$; if $ M^3 \ll \sqrt{\lambda} g m M_P^2$, then inflation ends within one $e$-fold of expansion after reaching $\phi_c$.
% The following parameter values offered in \cite{linde1994hybrid} result predictions that agree with observed features of the scalar density perturbation spectrum: 
% % \[ M \sim 10^{11} \text{ GeV} \qquad m \sim 10^2 \text{ GeV} \qquad g^2 \sim \lambda \sim 0.1 \]
% \[ M \sim 10^{-8} M_P \qquad m \sim 10^{-17} M_P \qquad g^2 \sim \lambda \sim 0.1 \]
%
% The regimes are denoted by the relation of $\phi$ to the dimensionless parameter $a \equiv M^4/2\lambda m^2$.  For $\phi \gg a$, the potential is mass dominated; for $\phi \ll a$, it is vacuum dominated.
%
Since the hybrid inflation potential exhibits no false vacua, we are left with the possibilities of stochastic and topological eternal inflation. 
If eternal inflation is found to occur for field values not far outside the range from which density perturbations are likely to have been imprinted, then it would be difficult to argue that eternal inflation is generically absent from the model.

\paragraph{Stochastic Eternal Inflation}

% Stochastic eternal inflation occurs when quantum fluctuations dominate the classical evolution of the inflaton.
% Over the passage of a Hubble time $H^{-1}$, $\phi$ decreases by an amount $\Delta \phi = \lvert\dot\phi\rvert H^{-1} = V_{,\phi} / 3H^2 $ due solely to its classical slow-roll evolution, while quantum fluctuations with amplitude $\delta\phi \approx H/2\pi$ may drive the field up or down the slope relative to that trajectory.  
% If in that time, the probability for the field within an initially Hubble-sized region to increase is greater than the ratio of initial to final volume ($1/e^3$), then at least one final Hubble volume is likely to continue inflating.  
% This occurs when $\Delta \phi \lesssim \delta \phi \, \sqrt{2} \, \erfc^{-1} (2e^{-3})$ or $ \delta\phi \gtrsim 0.61 \, \Delta\phi $.  
In the hybrid model, Eq.~\eqref{seic} is  equivalent to the constraint
\begin{equation} \phi \lesssim \frac{0.15 \, V^{3/2}}{M_P^3 \, m^2} \end{equation}
It is useful to identify in the domain of $\phi$ two regimes of approximation, in which the potential \eqref{valley} of the inflationary valley is dominated by either
the quadratic term $\frac12 m^2\phi^2$ ($\widebar\phi \gg a$) or
the vacuum term $M^4/4\lambda$ ($\widebar\phi \ll a$).
% By combining the following conditions, we find the constraints under which eternal inflation is allowed.
% \begin{enumerate}
% \item Slow roll conditions
%     \begin{enumerate}[label=\arabic{*}.]
%     \item $\epsilon_\phi = \dfrac{m^4\phi^2}{2V^2} \ll M_P^{-2}$
%     \item $\eta_\phi = \dfrac{m^2}{V} \ll M_P^{-2}$
%     \end{enumerate}
% \item Criterion for eternal inflation: $\phi \lesssim \dfrac{\widebar V^{3/2}}{\widebar m^2} \dfrac{M_P}{6.64} $
% \item Observed spectrum of density perturbations
%     \begin{enumerate}[label=\arabic{*}.]
%     \item 
\[ Q_s = \frac{m (\phi^2 + a^2 \, M_{\text P}^2)^{3/2}}{\pi \sqrt{600} \, M_P^3 \, \phi } = (1.945 \pm 0.052) \times 10^{-5} \]
%     \item $ n_s - 1 = \dfrac{2 m^2}{V} \left( 1 - \dfrac{3 \, m^2 \phi^2}{2 V} \right) M_P^2 = -0.047 \pm 0.016 $
%     \item $ \alpha_s = \dfrac{4 m^4 \phi^2}{V^2} \left( \dfrac{2 m^2}{V} - \dfrac{ 3 m^4 \phi^2}{2 V^2} \right) M_P^4 = -0.040 \pm 0.027 $
%     \end{enumerate}
% \end{enumerate}
% $ \alpha_s = \dfrac{4 m^4 \phi^2}{V^2} \left( \dfrac{2 m^2}{V} - \dfrac{ 3 m^4 \phi^2}{2 V^2} \right) M_P^4 = -0.040 \pm 0.027 $
% The quadratic approximation is $V(\phi,0) \approx \frac12 m^2 \phi^2$.
In the quadratic regime, the inflaton behaves like a free scalar field with mass $m$.  The slow roll conditions are satisfied when $\widebar\phi \gg 1$, and the criterion for eternal inflation is \[ \widebar \phi \gtrsim 4.3 \, \widebar m^{-1/2}.\] %Q_s \gtrsim 0.24 \]
In the regime $a \lesssim 1$, the field excursion during the last $\phi$ at 55 e-folds before the end of inflation asymptotes to approximately $14.8 \, M_P$ as $a \to 0$.  
For $\overline m \ll 1$ and $\widebar\phi_c \lesssim 1$, the field cannot satisfy the eternal inflation criterion within $10^{10}$ $e$-folds.
The parameters of the perturbation spectrum for $\phi \approx 14.8 \, M_P$ are given in Table \ref{quadtable}.
% { \def\arraystretch{2.1}
% \begin{table}[h]
% \centering
% \begin{tabular}{ccll}
%     Parameter   & Expression & $\widebar\phi \approx 14.8$ & Measured Value \\
%     $Q_s$       & $\dfrac{\widebar m \widebar \phi^2} {2\pi\sqrt{150}}$  &  $\phantom{-}2.8 \, \widebar m$  &  $(1.945 \pm 0.052) \times 10^{-5}$
% \\  $n_s - 1$   & $-8\,\widebar\phi^{-2}$               & $-0.036$         & $-0.047 \pm 0.016$
% \\  $\alpha_s$  & $-32\,\widebar\phi^{-4}$              & $-0.00067$       & $-0.040 \pm 0.027$
% \\  $r$         & $\phantom-64\,\widebar\phi^{-2}$      & $\phantom-0.29$  & $\phantom-0.2^{+0.07}_{-0.05}$
% \end{tabular} 
% \caption{Parameters of the density perturbation spectrum in the quadratic approximation.}
% \label{quadtable}
% \end{table} }

% \[ Q_s \approx \dfrac{ \widebar m \widebar \phi^2} {2\pi\sqrt{150} M_P^3} \approx 2.8 \widebar m \approx (1.945 \pm 0.052) \times 10^{-5} \]
% \[ n_s - 1 \approx -\dfrac{8 M_P^2}{\phi^2} \approx -0.047 \pm 0.016 \implies \phi_e \approx 13 M_P \]
% \[ \alpha_s \approx -\dfrac{32 M_P^4}{\phi^4} \approx -0.040 \pm 0.027 \implies \phi_e \approx 5 M_P \]
% \[ r = \frac{2^6 M_P^2}{\phi^2} \overset?< 0.30 \impliedby \phi > 15 M_P \]

% The vacuum approximation is $V(\phi,0) \approx \frac{M^4}{4\lambda}$.
In the vacuum approximation, the first and second slow roll conditions are, respectively, $\widebar\phi \ll a^2$ and $a^2 \gg 1$.
These are easily met, as they are essentially the conditions for the vacuum dominance approximation.  The criterion for eternal inflation is \[\widebar\phi \lesssim 0.053 \, \widebar m \, a^3.\]
Given $\widebar m \ll 1$ and $a \gg 1$, this too is easily satisfied, meaning that eternal inflation occurs for small field inflation in the vacuum dominated regime with $\sigma = 0$.
For $\phi > \phi_c$, the eternal inflation criterion implies a lower bound on the scalar density perturbation amplitude,
% \[ a \gg \widebar\phi_c \qquad a^2 \gg \widebar\phi_c \qquad a^3 \gtrsim \dfrac{\widebar \phi_c}{\widebar m} \]
\[ Q_s \gtrsim 0.25, \] %4 \times 10^{-3} \]
that is larger than the measured value by four orders of magnitude.
So we know that density perturbations must have been imprinted at $\phi < \phi_c$.  Not accounting for the effects of including $\sigma$, the amplitude would match for $\phi \approx 2.2 \times 10^{-5} \, \phi_c$.

In the regime $a \gg 1$, 55 e-folds affects almost no change in the field value, and we can approximate $\phi_0 \approx \phi_c$.  
The parameters of the perturbation spectrum are given in Table \ref{vactable}.

{ \def\arraystretch{1}
\begin{table}[h]
\centering
\begin{tabular}{|c|c|l|l|}
    \hline
    Parameter   & $\phi \approx \phi_c$ & Measured Value \\
    \hline
    $Q_s$       & $\dfrac{1} {2\pi\sqrt{150}} \dfrac{\widebar m \, a^3}{\widebar\phi_c}$  &  $(1.945 \pm 0.052) \times 10^{-5}$ \\
    \hline
    $n_s - 1$   & $\dfrac{1}{a} \left( 1 - \dfrac{12 \widebar\phi_c^2}{a} \right)$  &  $-0.047 \pm 0.016$ \\
    \hline
    $\alpha_s$  & $\dfrac{2^{4} \widebar\phi_c^2}{a^6} \left(1 - \dfrac32 \dfrac{\widebar\phi_c^2}{a^2} \right) $                   & $-0.040 \pm 0.027$ \\
    \hline
    $r$         & $\dfrac{32 \, \widebar\phi_c^2}{a^2}$  & $\phantom-0.2^{+0.07}_{-0.05}$ \\
    \hline
\end{tabular} 
\caption{Parameters of the scalar density perturbation spectrum in the vacuum approximation of hybrid inflation.}
\label{vactable}
\end{table} }

Neglecting motion in the $\phi$-direction, the slow roll conditions for $\sigma$ in the vacuum approximation are
\[ \lambda \widebar\sigma \abs{\eta^2 - \widebar\sigma^2} \ll \widebar m^2 a^2 \quad\text{and}\quad \lambda \abs{\eta^2 - 3\widebar\sigma^2} \ll \widebar m^2 a^2,\]
where $\eta \equiv \widebar M/\sqrt{\lambda}$.
\[ Q_s \approx \dfrac{g} {8\pi\sqrt{75} \, \lambda^{3/2}} \dfrac{ \widebar M^5 }{ \widebar m^2 } \approx (1.945 \pm 0.052) \times 10^{-5} \]
% \[ n_s - 1 \approx \dfrac{2\lambda \widebar m^2}{\widebar M^4} \left( 1 - \dfrac{24 \lambda m^2}{g^2 M^2} \right) \approx -0.047 \pm 0.016 \]
% \[ \alpha_s \approx \dfrac{2^{10} \lambda^3}{g^2} \dfrac{\widebar m^6}{\widebar M^{10}} \left(1 - \dfrac{3 \lambda }{2 g^2} \dfrac{\widebar m^2}{\widebar M^2} \right) \approx -0.040 \pm 0.027 \]
% \[ r = \frac{2^8 \lambda^2 M_P^2 \, m^4 \phi^2}{M^8} \overset?< 0.30 \impliedby \phi < \frac{\widebar M^4}{\widebar m^2} \frac{M_P}{30\lambda} \]

% \paragraph{Number of e-folds}

The number of $e$-folds of inflation, $\Ne$, elapsed since the imprinting of CMB density perturbations is between 50 and 60, with 55 being an acceptable figure.  
Reversing the integral expression for $N$ yields a differential equation for $\phi(N)$:
\[ \ddx{\widebar \phi}{\Ne} = \frac{ 2 \widebar \phi }{ \widebar \phi^2 + a^2 } \]
The initial value $\phi_0$ from which the descent to $\phi_c$ produces $N$ $e$-folds of inflation is
\[ \widebar\phi_0^2(\Ne) = a^2 \, W \left[ \frac{\widebar \phi_c^2}{a^2} \exp \left(\frac{ 4 \Ne + \widebar\phi_c^2 }{a^2} \right) \right], \]
where $W(z)$ is the product logarithm (defined such that $\phi_0(0) = \phi_c$).  
For any $\phi_c < M_P$, there exists a threshold near $\Ne \sim a^2$ at which $\phi_0(\Ne)$ changes from $\ll M_P$ to $> M_P$, as shown in the figure below.  
% When $\widebar\phi \gtrsim a$, $\phi$ becomes linear in $a$ and $N$.

In Figure~\ref{hybrid_Ne}, we see coincidence among the initial field value $\phi_0$, the parameter $a$, and the number of $e$-folds $\Ne$.
The shaded region is excluded by the scalar spectral index.
The green regions are where stochastic eternal inflation occurs.  Why is there a green region in the small $e$-fold regime at the boundary of the shaded region?

\begin{figure}[h]
    \centering
    \includegraphics[width=8cm]{Figures/phi0_vs_a_N_Eternal_Region}
    \caption[Stochastic Inflation in Hybrid Models]{Surface of coincidence among the parameter $a$, the initial field value $\phi_0$, and the number of $e$-folds $\Ne$ in the hybrid inflation model \eqref{hybrid_potential}.  Regions with stochastic eternal inflation are colored green.  The white line denotes $\Ne = a^2$.  The shaded region is excluded by the measurements of the scalar spectral index.}
    \label{hybrid_Ne}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=10cm]{Figures/RegionPlot_a_N_phi0}
\end{figure}

\paragraph{Topological Eternal Inflation}

For $\phi < \phi_c$, the potential has two local minima at $\pm M/\sqrt{\lambda}$.  
In neighboring regions of space that begin with $\sigma$ near its local maximum, the field can roll down the slope in different directions -- toward $-M/\sqrt{\lambda}$ or $+M/\sqrt{\lambda}$.  
This leads to the formation a domain wall in which the field is stuck near the local maximum.  
If the potential near the maximum is sufficiently flat, so that the domain wall thickness exceeds the Hubble radius, then the volume within the wall will inflate faster than it decays.
\[ \left. \ddx{^2V}{\sigma^2} \right\rvert_{\sigma=0} \ll \frac{V}{3 M_P^2} \]
\[ g^2 \phi^2 - M^2 \ll \frac{1}{3 M_P^2} \left( \frac{M^4}{4\lambda} + \frac{m^2}{2} \phi^2 \right) \]
\[ \left( g^2 - \frac{4\pi}{3} \, \widebar m^2 \right) \phi^2 \ll \left( 1 + \frac{2\pi}{3} \frac{\widebar M^2}{\lambda} \right) M^2 \]
If $\widebar m \ll 1$ and $\widebar M^2 \ll \lambda$, then the potential is sufficiently flat for $\phi \ll \phi_c$.  

We must also assert that the kinetic energy of $\phi$ be sub-dominant -- satisfying the slow roll conditions.  The two can be consistent if the potential is vacuum dominated:
\[ \phi \ll \frac{\widebar M^4}{\widebar m^2} \frac{M_P}{\lambda} \qquad \widebar M^4 \gg \lambda \widebar m^2 \]

\[\widebar m = 1 \quad \widebar m = 10^{-5} \quad \widebar m = 10^{-10} \]

\[ \log_{10} \frac{\widebar\phi_0}{a} = 0 \quad \log_{10} \frac{\widebar\phi_0}{a} = -2 \quad \log_{10} \frac{\widebar\phi_0}{a} = 4 \]


    \[ n_s - 1 = \dfrac{2 m^2}{V} \left( 1 - \dfrac{3 \, m^2 \phi^2}{2 V} \right) M_P^2 = -0.047 \pm 0.016 \]
    \[ \alpha_s = \dfrac{4 m^4 \phi^2}{V^2} \left( \dfrac{2 m^2}{V} - \dfrac{ 3 m^4 \phi^2}{2 V^2} \right) M_P^4 = -0.040 \pm 0.027 \]


==> Trash/251proj.tex <==

\subsection{Exterior Algebras}
Equipping a vector space with the {\it exterior product} allows one to construct an oriented geometric extent of any dimension up to the the number of dimensions of the original vector space.  The exterior product is denoted by the wedge ($\wedge$) operator, and is bilinear and antisymmetric in its two arguments
\[ \mathbf e_i \wedge \mathbf e_j = -\mathbf e_j \wedge \mathbf e_i \]
% \vspace{.3cm}
The number of vector elements in the exterior product is identified as the {\it grade}.
An element consisting of contributions from a single grade $k$ is known as a blade (or $k$-blade).
A 0-blade is a scalar; a 1-blade is a vector, and so on.
If the original vector space is $\mathbb R^n$, a multivector of grade 1, or simply a vector, represents an oriented length ($\mathbf a = a_i \, \mathbf e_i \in \mathbb R^n $).  
A \emph{bivector} of grade 2 is an oriented area ($\mathbf a \wedge \mathbf b = a_i b_j \, \mathbf e_i \wedge \mathbf e_j \in \bigwedge \mathbb R^n$).
And generally an oriented $k$-vector is an element of the vector space
\[ \mathbf e_1 \wedge \mathbf e_2 \wedge \cdots \wedge \mathbf e_k \in \bigwedge^{k-1} \mathbb R^n \]
% \end{description}}
A vector space of dimension $n$ equipped with the exterior product generates an {\it exterior algebra} of dimension $2^n$.
\[ \textstyle \Lambda \!\left(\mathbb R^n\right) = \mathbb R \oplus \mathbb R^n \oplus \bigwedge \mathbb R^n \oplus \bigwedge^2 \mathbb R^n \oplus \cdots \oplus \bigwedge^{n-1} \mathbb R^n \]
The volume element used in integration in an $n$-dimensional space is an $n$-blade: $\dx V = \dx x^1 \wedge \dx x^2 \wedge \cdots \wedge \dx x^n$


\subsection{Clifford Algebras}
Let $V$ be equipped with a symmetric inner product mapping two elements of $V(\mathbb K)$ to the underlying field $\mathbb K$, of the form $\mathbf a \cdot \mathbf b = \frac12 \left( Q(\mathbf{a+b}) - Q(\mathbf a) - Q(\mathbf b) \right)$ for some quadratic form $Q$.
Joining this inner product with the exterior product produces the Clifford product:
\[ \qquad\;\, \mathbf{ab} = \mathbf a \cdot \mathbf b + \mathbf a \wedge \mathbf b\]
\vspace{.2cm}
Equipping such an inner product space over a field $\mathbb K$ with the Clifford product generates a {\it Clifford algebra} $C\ell_n(\mathbb K)$, which is an exterior product space: $C\ell_n(\mathbb K) \to \bigoplus_{i=0}^n \bigwedge^i V$,

Further equipping the Clifford algebra with a norm defined as the inner product of an element with itself
\[ \abs{\mathbf a} = \sqrt{\langle \mathbf a \mathbf a \rangle_0} \]
every Clifford algebra is a composition algebra satisfying $\lvert \mathbf{ab} \rvert^2 = \lvert \mathbf a \rvert^2 \lvert \mathbf b \rvert^2 $, and has a set of privileged orthogonal bases for which
\[ \mathbf e_i \mathbf e_i = Q(e_i)1 \qquad \mathbf e_i \mathbf e_j = -\mathbf e_j \mathbf e_i \mid i \neq j \]
% \end{itemize} \vspace{.2cm}
We can define the {\it Hodge dual} of any multivector by multiplying it by a unital element of the largest grade
\[ \star \mathbf a = \mathbf a \prod_{i=1}^n \mathbf e_i \]
In three dimensions, the Hodge star is a one-to-one map between vectors to bivectors.
\[ \mathbf e_i \mathbf e_j + \mathbf e_j \mathbf e_i = \delta_{ij} \]

\subsection{Geometric Algebras}
A Clifford algebra over $\mathbb R^n$ is a {\it geometric algebra}.
For example, a generic element of $C\ell_2(\mathbb R)$ takes the form 
\[ \mathbf a = a_0 + a_1 \mathbf \sigma_1 + a_2 \mathbf \sigma_2 + a_{12} \mathbf \sigma_1 \mathbf \sigma_2 \]
\begin{table}[h]
\centering
    \begin{tabular}{c|ccc}
        1                   & $\sigma_1$            & $\sigma_2$            &   $\sigma_1 \sigma_2$ \\ \hline
        $\sigma_1$          & 1                     & $\sigma_1 \sigma_2$   &   $\sigma_2$          \\
        $\sigma_2$          & $-\sigma_1 \sigma_2$  & 1                     &   $-\sigma_1$         \\
        $\sigma_1 \sigma_2$ & $-\sigma_2$           & $\sigma_1$            &   $-1$                \\
    \end{tabular}
\end{table}
The even sub-algebra -- spanned by the Clifford products of an even number of vector elements -- for the geometric algebra $\mathcal C \ell_2(\mathbb R)$ is isomorphic to the complex numbers, while the even subalgebra of $\mathcal C \ell_3(\mathbb R)$ is the quaternions.
\[ C\ell_2^+(\mathbb R): \{1,\sigma_1 \sigma_2\} \mapsto \mathbb C \qquad C\ell_3^+(\mathbb R): \{1,\sigma_1 \sigma_2, \sigma_2 \sigma_3, \sigma_3 \sigma_1\} \mapsto \mathbb H \]
The Pauli matrices provide representations of $C\ell_2(\mathbb R)$ and $C\ell_3(\mathbb R)$: $\sigma^i \sigma^j + \sigma^j \sigma^i = 2 \delta^{ij}$
\[ \sigma_1 = \begin{pmatrix} 0 & 1 \\ 1 & 0 \end{pmatrix} \quad \sigma_2 = \begin{pmatrix} 0 & -i \\ i & 0 \end{pmatrix} \quad \sigma_3 = \begin{pmatrix} 1 & 0 \\ 0 & -1 \end{pmatrix} \]

\chapter{Spinors}

\subsection{$C\ell_3(\mathbb R)$ in the Schrodinger-Pauli Equation}
The Shr\"odinger-Pauli equation takes the form
\[ \displaystyle i \pdx{\psi}{t} = \frac{\hat\pi^2}{2m} \psi + e \phi \psi \]
If we identify the momentum operator with $\pi_i = \partial_i - i e A_i$, then a straightforward interpretation of this equation might be
\[ i \pdx{\psi}{t} = \frac1{2m} \left[ ( -i\nabla - e \mathbf A ) \cdot ( -i\nabla - e \mathbf A ) \right] \psi + e \phi \psi \]
where the square denotes the 3-vector dot product.  Since the dot product is not an algebraic product (it does not map elements of a vector space to an element of the same space), it ends up ``throwing away geometric information.''  
% We can resolve this shortcoming by promoting the 3-vectors $\nabla$ and $\mathbf A$ to vector elements of $C\ell_3(\mathbb R)$: $\nabla \to \fslash \partial = \sigma^i \partial_i$.
% \[ i \pdx{\psi}{t} = \frac1{2m} (-i \fslash \partial - e \fslash A)^2 \psi + e \phi \psi \]
Since the components do not commute, the exterior product of $\partial$ and $\mathbf A$ gives the magnetic term
\begin{gather*}
    \left( i\fslash\partial + e \mathbf A \right) \cdot \left( i\fslash\partial + e \mathbf A \right) = -\nabla^2 + i e ( \fslash\partial \cdot \mathbf A + \mathbf A \cdot \nabla) + e^2 A^2 \\
    \left( i\fslash\partial + e \mathbf A \right) \wedge \left( i\fslash\partial + e \mathbf A \right) = - e \epsilon^{ijk} (\partial_i A_j) \sigma_k = - e \fslash B
\end{gather*} 
producing the coupling of a spin magnetic moment to an external magnetic field.

\subsection{Spinors}%{Why projections?}
% \begin{minipage}{0.7\textwidth}
The components of a Weyl spinor can be thought of in terms of a stereographic projection from the pole of the unit sphere onto the plane passing through the origin.  If the coordinates of the projected point are $(x,y)$, the complex representation of that point can be identified with the ratio of the two spinor components, given the constraint that the norm of the spinor is 1.
\[ \zeta = x + iy \equiv {\psi_2}/{\psi_1} \qquad \psi_1 \psi_1^* + \psi_2 \psi_2^* = 1 \]
% \[ \zeta' = (1 + i\theta) (x + iy) \equiv \frac{\psi_2}{\psi_1} \]
The coordinates of the original point on the unit sphere can then be reconstructed as
\[ x = \psi_1 \psi_2^* + \psi_1^* \psi_2 \quad y = i (\psi_1 \psi_2^* + \psi_1^* \psi_2) \quad z = \psi_1 \psi_1^* - \psi_2 \psi_2^* \]
Under an infinitesimal rotation carried out in the projection plane, that complex number transforms as
\[ \frac{\psi_2'}{\psi_1'} = (1 + i\theta) \frac{\psi_2}{\psi_1} = \frac{(1 + i\theta/2)\psi_2}{(1 - i\theta/2)\psi_1} \to \frac{e^{+i\theta/2} \,\psi_2}{e^{-i\theta/2} \,\psi_1} \]
% \end{minipage}
% \begin{minipage}{0.27\textwidth}
%     \includegraphics[width=3.7cm]{SpinProjection}
% \end{minipage} \vspace{-.2cm}
% {\sout{What are they?}  Better question: What do they {\it do}?}
implying that a rotation of $2\pi$ radians results in a negative sign on the spinor components. 
Spinors $(\psi_1,\psi_2)$ are elements of a complex projective space $\mathbb{CP}^{n}$.
% , labeling lines through the origin of the complex vector space $\mathbb C^{n}$.  
% \begin{description}[leftmargin=!,labelwidth=2.8cm]
The inner product of a spinor sandwiching a vector element of the geometric algebra amounts to a projection of that element onto the direction identified by the spinor.
% \[ \psi^\dag \fslash a \psi = \Tr {\psi \psi^\dag \fslash a} = \vec a \cdot \hat \xi\]
, for some $\hat \xi $
The quantity $\psi^\dag \vec \sigma \psi$ transforms with $\mathrm{SO}(3)$, and  
$\psi$ transforms with $\mathrm{Spin}(3) \cong \mathrm{SU}(2)$, the double cover of $\mathrm{SO}(3)$.



\subsection{Spin Groups}
A spin group is a double cover of the corresponding special orthogonal group $\mathrm{SO}(p,q)$ of distance-preserving transformations in a space with signature $p{+}q$.
% \begin{description}[leftmargin=!,labelwidth=2.1cm]
The Lie group is \[ \mathrm{Spin}(p,q) = \{ s \in C\ell_{p,q}(\mathbb R) \mid s^\dag s = 1, \, \bar s s = 1 \} \]
The Lie algebra is the subalgebra of {bivectors}: $S^{ij} = \frac14 \, [\sigma^i, \sigma^j] = \frac12 \, \sigma^i \wedge \sigma^j$
    % \vspace{.2cm}
    \hfil $ [S^{ij},\, S^{k\ell}] = S^{i\ell} \eta^{jk} + S^{jk} \eta^{i\ell} - S^{ik} \eta^{j\ell} - S^{j\ell} \eta^{ik} $
    % \vspace{.2cm}
Rotations $\mathbb R^{p+q} \to \mathbb R^{p+q} : \mathbf x \rightarrow \mathbf x' = s \mathbf x \bar s$
% \end{description}
% \begin{minipage}{0.6\textwidth}
\[
\mathrm{Spin}(3) \cong \mathrm{SU}(2) \quad
\mathrm{Spin}(4) \cong \mathrm{SU}(2) \otimes \mathrm{SU}(2) \quad
\mathrm{Spin}(1,3) \cong \mathrm{SL}(2,\mathbb C) \]
% \end{minipage}
% \begin{minipage}{0.37\textwidth}
% \begin{figure}
%     \includegraphics[width=4.5cm]{SO3_Homotopy}
% \end{figure}
% \end{minipage}



\subsection{Algebra of Physical Space}
When describing null four-vectors in the tangent space on a Lorentzian manifold, we can identify the temporal component with the scalar identity element.  Defining two sets of bases
\[ \sigma^\mu \equiv (I_2, +\vec\sigma) \quad \bar\sigma^\mu \equiv (I_2, -\vec\sigma) \]
A null four-vector with components $x_\mu$ then takes the form
\[ \sigma^\mu x_\mu \equiv x_0 + \vec x \cdot \vec \sigma = \begin{pmatrix} x_0 + x_3 & x_1 - ix_2 \\ x_1+ix_2 & x_0-x_3 \end{pmatrix} \]
{\bf Lorentz Transformations} \hspace{.1cm} $\mathrm{SO}(1,3) \mapsto \mathrm{Spin}(1,3) \cong \mathrm{SL}(2,\mathbb C)$  
\[ \chi^\dag \sigma^\mu x_\mu \chi \to \chi^\dag \exp\left( -\tfrac i2 \omega_{\mu\nu} S^{\mu\nu} \right) \sigma^\mu x_\mu \exp\left(\tfrac i2 \omega_{\mu\nu} S^{\mu\nu} \right) \chi \]
The Lie algebra is the subalgebra of biparavectors: 
$S^{\mu\nu} = \frac12  \expv{\sigma^\mu \bar\sigma^\nu}_V $
\[ S^{0i} = -\tfrac12 \sigma^i = K^i \qquad S^{ij} = -\tfrac i2 \epsilon_{ijk} \sigma^k = \epsilon_{ijk} J^k \]
This allows us to factorize the massless Klein-Gordon equation
\[ \partial^\mu \partial_\mu \chi = 0 \implies \sigma^\mu \partial_\mu \chi = 0 \]
Inequivalent representations $\sigma^\mu$ and $\bar\sigma^\mu$: $\left(\tfrac12,0\right)$ and $\left(0,\tfrac12\right)$
% \[ \text{ Two-component Weyl spinors:} \quad \chi \to \exp\left(\tfrac12 \omega_{\mu\nu} S^{\mu\nu} \right) \chi \]
% What happens when we add mass?

\subsection{Chirality}
\[ \sigma^\mu \to S \sigma^\mu S^\dag \]
\[ \mathcal L = i \psi^\dag \sigma^\mu \partial_\mu \psi \]

\subsection{Spacetime algebra $C\ell_{1,3}(\mathbb C)$ and the Dirac Equation}
The algebra $\mathcal C\ell_3(\mathbb R)$ can only represent null four-vectors.
\[ -\hbar^2 \partial^\mu \partial_\mu \psi = m^2 \psi \;\to\; i \gamma^\mu \partial_\mu \psi = i \fslash\partial \psi = m \psi \]
In the relativistic theory, mass comes to occupy the scalar term, as it is invariant under the largest set of propor transformations.  Meanwhile, the temporal component of the 4-vector is associated to a vector element $\gamma^0$.
To mix positive and negative frequencies, we need $\left(\tfrac12,0\right) \oplus \left(0,\tfrac12\right)$. %two copies of $C\ell_3(\mathbb R)$
% \begin{align*}
%     S^{\mu\nu} &= \frac14 \begin{pmatrix} 
%     0 & i\sigma_1 \otimes \sigma_2\sigma_1 & i\sigma_2 \otimes \sigma_2\sigma_1 & i\sigma_3 \otimes \sigma_2\sigma_1 \\
%     i\sigma_1 \otimes \sigma_1\sigma_2     & 0 & -\sigma_1\sigma_2 \otimes I_2  & -\sigma_1 \sigma_3 \otimes I_2 \\
%     i\sigma_2 \otimes \sigma_1\sigma_2     & -\sigma_2 \sigma_1 \otimes I_2 & 0 & -\sigma_2 \sigma_3 \otimes I_2 \\
%     i\sigma_3 \otimes \sigma_1\sigma_2     & -\sigma_3 \sigma_1 \otimes I_2     & -\sigma_2 \sigma_3 \otimes I_2 & 0 \\
% \end{pmatrix} \\
% S^{\mu\nu} &\equiv \frac12 \, \gamma^\mu \wedge \gamma^\nu \implies \gamma^0 = I_2 \otimes \sigma_1, \quad \gamma^k = i\sigma_k \otimes \sigma_2
% \end{align*}
\[ \gamma^\mu \gamma^\nu + \gamma^\nu \gamma^\mu = 2 \eta^{\mu\nu} I_2 \otimes I_2 \]

In the chiral representation, the gamma matrices take the form
\[ \gamma^\mu = \begin{pmatrix} 0 & \bar\sigma^\mu \\ \sigma^\mu & 0 \end{pmatrix} \]
where $\sigma^\mu \to S^\dag \sigma^\mu S$ and $\bar\sigma^\mu \to S \bar\sigma^\mu S^\dag$ are the vector elements of two Clifford algebras with the opposite orientation.
The Lagrangian producing the Dirac equation is
\[ \mathcal L_{\text{Dirac}} = i \bar\psi \gamma^\mu (\partial_\mu - i e A_\mu) \psi - m \bar\psi \psi \]
where $\bar\psi \equiv \psi^\dag \gamma^0$ and, in the chiral representation, 
\[ \psi = \begin{pmatrix} \psi_L \\ \psi_R \end{pmatrix} \]

% \vspace{2cm}
% \begin{minipage}{8cm}
% \noindent Whatever the dark matter turns out to be, let's just agree to denote it with the symbol $\hat W$.  Then we can stop asking, ``What is the dark matter?''; the answer is always ``Yes.''
% \end{minipage}
% \vspace{2cm}
% \begin{thebibliography}{10}

% \beamertemplatebookbibitems
% % Start with overview books.

% \bibitem{Lounesto} P.~Lounesto.  {\em Clifford Algebras and Spinors, Second Edition}.  Cambridge University Press.  (2001)

% \bibitem{Hladik} J.~Hladik.  {\em Spinors in Physics}.  Springer Science and Business Media.  (2012)

% \bibitem{Wald} R.M.~Wald.  ``Spinors.''  {\em General Relativity}.  The University of Chicago Press.  (1984)
% \end{thebibliography}
% \end{frame}


==> Trash/covariance.tex <==
% % \subsection{Mechanics and Covariance}
% Consider a multivector field $\mathcal F$ consisting of a scalar part (proportional to $\varsigma^0$) and bivector parts ($\varsigma^i, \, \varsigma^j \varsigma^k $), and transforming as
% $ \mathcal F \to S \mathcal F S^{-1} $, where 
% $S = \exp {(\frac12 w_i \varsigma^i + \frac 14 \epsilon_{ijk} \theta_{i} \varsigma^j \varsigma^k)}$ defines a Lorentz transformation.  
% If the bivector part corresponds to the field strength tensor for electromagnetism, then a space-time split divides those degrees of freedom into the electric polar vector $\mathbf E$ and the magnetic axial vector $\mathbf B$.  
% % In the free theory, $\mathbf E$ and $\mathbf B$ enter symmetrically into the equations of motion, and those equations are reduced to three.  This reduction in meaningful degrees of freedom allows us to derive the equations of motion from a first-order Lagrangian.
% \[ \mathcal F = \varsigma^j E_j + \tfrac12 \epsilon_{ijk} \varsigma^i \varsigma^j B_k 
% = {\textstyle \sum_j \varsigma^j (E^j + i B^j)} \]
% % \[ S_{jk} = \cos \tfrac\theta2 + \varsigma^j \varsigma^k \sin \tfrac\theta2 \]
% % \[ S_{0i} = \cosh \tfrac\eta2 + \varsigma^i \sinh \tfrac\eta2 \]
% % \[ \mathcal F \to S \mathcal F S^{-1} \]
% % \[ \Tr {\mathcal F^2} \to \Tr {S \mathcal F S^{-1} S \mathcal F S^{-1}} = \Tr{\mathcal F^2 S^{-1} S} = \Tr {\mathcal F^2} \]
% Presuming the existence of a vector gauge field $\mathbf A$ and asserting the identity $\mathbf F = \mathrm d \mathbf A$, the Lagrangian in terms of the vector potential takes the Yang-Mills form
% \[ \mathcal L(\partial A_\mu) = -\tfrac14 F_{\mu\nu} F^{\mu\nu} = -\tfrac12 A_{[\mu,\nu]} A^{[\mu,\nu]} \]
% Varying with respect to the vector potential $A_\mu$ yields the inhomogeneous Maxwell equations in terms of $A_\mu$. 

% If we instead express this Lagrangian in terms of the measurable quantities $\mathbf E$ and $\mathbf B$ and vary with respect to them, then we find for the classical equations of motion
% \[ \mathcal L(\mathbf E, \mathbf B) \equiv \tfrac12 (\mathbf E \cdot \mathbf E - \mathbf B \cdot \mathbf B) \implies \mathbf E = \mathbf B = 0 \]
% The justification for this result is that the underlying gauge field represents the true degrees of freedom, and that the 6 degrees of freedom contained in $\mathbf E$ and $\mathbf B$ are over-counted and cannot be varied independently.
% However, consider the modified Lagrangian
% \begin{equation} \mathcal L(A_\mu,\mathcal F,\partial\mathcal F) = { \textstyle  \Tr { \varsigma^\mu \varsigma^\rho A_\mu \partial_\rho \mathcal F } } - \tfrac14 \Tr {\mathcal F^2} + {\text{h.c.}} \label{eq:lagrangianpsiAF} \end{equation}
% where $A_\mu$ and $\mathcal F$ are taken to be independent variables.
% % The middle term is Lorentz invariant under transformation of $\varsigma^\mu A^\mu \to S \varsigma^\mu A^\mu S^\dag$ and $\mathcal F(\mathbf x) \to S \mathcal F(\mathbf \Lambda^{-1}\mathbf x) S^{-1}$.
% % \[ \sum_\mu \varsigma^\mu \!A^\mu \varsigma^\nu \partial_\nu \mathcal F \to 
% % \sum_\mu (S \varsigma^\mu \!A^\mu S^\dag) \varsigma^\nu \partial_\nu (S \mathcal F S^{-1}) =
% % \sum_\mu \varsigma^\mu \!A^\mu (S^\dag \varsigma^\nu S) \Lambda_\nu^{\phantom\nu\rho} \partial_\rho \mathcal F \]
% Varying with respect to $A_\mu$ yields the inhomogeneous Maxwell equations in terms of $\mathbf E$ and $\mathbf B$, 
% % \begin{align*}
% % \tfdx{S}{A_0} &= \nabla \cdot \mathbf E \\
% % \tfdx{S}{\mathbf A} + \mathbf E &= \nabla \times \mathbf B
% % \end{align*}
% while varying with respect to $\mathcal F = \varsigma^j(E_j + i B_j)$ yields the definitions of those fields in terms of $A_\mu$.
% \begin{alignat*}{7}
% \tfdx{S}{A_0} &= \nabla \cdot \mathbf E - \psi^\dag \psi \\ 
% \tfdx{S}{\mathbf E} + \mathbf E &= \partial_0 \mathbf A - \nabla \! A_0 && \\
% \tfdx{S}{\mathbf A} + \dot {\mathbf E} &= \nabla \times \mathbf B + \psi^\dag \mathbf\varsigma \psi \\
% {-\tfdx{S}{\mathbf B}} + \mathbf B &= \nabla \times \mathbf A &&
% \end{alignat*}
% In this formulation, the gauge field serves as connective tissue coupling the spinor field $\psi$ to the bivector field $\mathcal F$, rather than a dynamical field standing on its own. Since no derivatives of $\mathcal A$ appear in the Lagrangian, we can think of $\mathcal A(x)$ as a Lagrange multiplier. 

% In the resulting free theory, we no longer have a use for the gauge field in describing the dynamics of $\mathcal F$, since $\mathcal F$ is gauge-invariant and there is no longer a coupling with the spinor field.  
% Unlike in the minimally coupled theory, the phase of $\mathcal F$ in the free theory is unobservable; there is no meaningful distinction between $\varsigma^j( E_j + i B_j)$ and $\varsigma^j( i E_j - B_j)$.

% We should be able to cut out the middle man, eliminating $A_\mu$ and replacing the augmented Yang-Mills Lagrangian with one that is first-order and bilinear in $\mathcal F$.

\chapter{Geometric Algebra}

\input{Trash/251proj}

\chapter{On the Geometric Origin of Particle Species}

\subsection{First Order Formulations of Vector Field Theories}

\subsection{Electroweak Interaction}
For each generation of leptons, the left- and right-chiral components are
\[ \psi_L = \begin{pmatrix} e_L \\ \nu \end{pmatrix} \qquad \psi_R = e_R \]
where each of $e_L, e_R, \nu$ are Weyl spinors. 
\[ \mathcal L = i \psi_R^\dag \sigma^\mu \partial_\mu \psi_R + 
i \psi_L^\dag (I_2 \otimes \bar\sigma^\mu) \partial_\mu \psi_L \] 
Under rotations, Weyl spinors belonging to the two chiralities transform with different representations of the Lorentz group, related by Hermitian conjugation
\[ e_R(\mathbf x) \to S e_R(\Lambda^{-1} \mathbf x) \qquad e_L(\mathbf x) \to S^* e_L(\Lambda^{-1} \mathbf x) \qquad \nu(\mathbf x) \to S^* \nu(\Lambda^{-1} \mathbf x) \]
Under a global physical rotation, we have
\[ \mathcal L(\mathbf x) \to i \psi_R(\Lambda^{-1} \mathbf x)^\dag S^\dag \sigma^\mu S \partial_\mu \psi_R(\Lambda^{-1} \mathbf x) + 
i \psi_L(\Lambda^{-1} \mathbf x)^\dag (I_2 \otimes (S \bar\sigma^\mu S^\dag)) \partial_\mu \psi_L(\Lambda^{-1} \mathbf x) \]

At present, there is no compelling theoretic justification for fields of one chirality to belong to a doublet and those of the other to comprise singlets.  
The situation gets even more troubling when considering quarks, in which both components of the doublet have corresponding right-chiral partners, each comprising a singlet.
If any explanation can be cited as the standard one, it is circular observation that
the Lagrangian is symmetric under $SU(2)$ gauge transformations because the electron and neutrino form a doublet; and the electron and neutrino form a doublet because the Lagrangian is symmetric under $SU(2)$ transformations.
That the difference is based entirely on chirality, which is all about how the system behaves under rotations, suggests that an underlying geometric explanation should eventually prevail.

The Lagrangian is invariant under the global transformation $\psi_L \to (U \otimes I_2) \psi_L$.  Gauging the $SU(2)$ symmetry requires that we introduce a new covariant derivative for left-chiral fields, involving a new vector field $W_\mu$.
\[ \mathcal L = i \psi_R^\dag \sigma^\mu (\partial_\mu - 2i g' B_\mu) \psi_R + 
i \psi_L^\dag \left( (I_2 \otimes \bar\sigma^\mu) (\partial_\mu - i g' B_\mu) - i g (\hat T^a \otimes \bar\sigma^\mu) W^a_\mu \right) \psi_L \]
where the .  In the adjoint representation
\[ \hat T^a = \tfrac12 \sigma^a \]
\[ W_\mu = \sum_a W^a_\mu T^a \]
The transformation group for $B_\mu$ is $U(1)$, while that of $W_\mu$ is $SU(2)$.
\[ B_\mu \to B_\mu + \frac 1{g'} \partial_\mu \lambda \]
% \[ W_\mu \to U^\dag W_\mu U - i U^\dag \partial_\mu U \]
The new rules for the $SU(2)$ gauge transformation are
\[ \psi_L \to (U \otimes I_2) \psi_L \qquad W_\mu \to U W_\mu U^\dag - \tfrac ig U^\dag \partial_\mu U \]
for some unitary operator $U = \exp(\frac i2 \alpha_a \hat T^a)$.
This of course pulls apart the two chiral representations hidden in the gamma matrices, suggesting that treating spinors as representing geometric objects in a four-dimensional tangent space is not the right way.

\[ W_{\mu\nu} = (\partial_\mu W_\nu - \partial_\nu W_\mu) - i g \left[ W_\mu, W_\nu \right] \]
\[ \mathcal L = i \psi_R^\dag \sigma^\mu D_\mu \psi_R + i \psi_L^\dag \sigma^\mu \mathcal D_\mu \psi_L - \psi_L^\dag \phi \psi_R - \frac14 B_{\mu\nu} B^{\mu\nu} - \frac14 W_{\mu\nu} W^{\mu\nu} + \mathcal L_\phi \]
The generator for the unbroken $U(1)$ symmetry is
\[ Q = \tfrac12 \hat Y + \hat T_3 \]

\subsection{Geometric Algebra and Gauge Theories}

% \hspace{9pt} 
Two separate transformations are involved in implementing a change of reference frames: 
one of the coordinates and another of the basis vectors spanning the tangent space $T_p$ at each event $p$. 
A coordinate transformation changes the mapping between field values -- abstract geometric objects with properties independent of the reference frame in which they are described -- and the numbers labeling events on the manifold.
A basis transformation, on the other hand, changes the numbers we use to describe the abstract field value as a linear combination of basis vectors.
% The vector described by the pair of basis and components is an abstract geometric object that exists independently of a reference frame, but any relation of that abstract entity to data in the real world requires a choice of basis.
Given one or more functions $F_i(\mathbf x)$ identifying components $i$ of the value of the field $F$ at the event labeled by $\mathbf x$, we enact a coordinate transformation by changing the input to that function, and a basis transformation by linearly combining the outputs of the functions $F_i$ for the same input.
%
Under the two transformations, a Weyl spinor field $\psi$ for example transforms as
% Coordinate transformations change the mapping between field values and numbers labeling points on the manifold; while in a basis transformation, it is the numbers representing field values as linear combinations of vectors in the local tangent space that change. %, while the coordinates addressing field values remain constant.
\[ \psi(\mathbf x) \to \begin{cases}
S \psi(\mathbf x) & \text{(basis)} \\
\psi(\Lambda^{-1} \mathbf x) & \text{(coordinates)}
\end{cases} \]

Coordinate and basis transformations are almost always acted together, since in most cases it is simplest to adopt the holonomic basis, specified everywhere by $\partial/\partial x_\mu$. This aligns the basis vectors with the directions along which one coordinate increases while the others remain constant.

The notion of separability of coordinate and basis transformations described above is challenged when we are faced with the question of how a gauge field should transform under each class of transformations.
Under just a coordinate transformation, the Weyl Lagrangian becomes
\[ \mathcal L(\mathbf x) \to \mathcal L'(\mathbf x) = i \psi(\Lambda^{-1} \mathbf x)^\dag e^{-i \lambda(\Lambda^{-1} \mathbf x)} \sigma^\mu (\partial_\mu - i e A'_\mu(\Lambda^{-1} \mathbf x) ) e^{i \lambda(\Lambda^{-1} \mathbf x)} \psi(\Lambda^{-1} \mathbf x) \]
where $A'_\mu(\Lambda^{-1} \mathbf x)$ is the gauge and coordinate transformed version of $A_\mu(\mathbf x)$ to be determined.  
% A gauge transformation a gauge transformation, we obtain
% \[ \mathcal L'(\mathbf x) = i \psi(\mathbf x)^\dag e^{-i \lambda(\mathbf x)} \sigma^\mu (\partial_\mu - i e A_\mu - i \partial_\mu \lambda(x)) e^{i \lambda(\mathbf x)} \psi(\mathbf x) \]
% \[ \mathcal L'(\mathbf x) = i \psi(\mathbf x)^\dag e^{-i \lambda(\mathbf x)} \sigma^\mu (\partial_\mu + i \partial_\mu \lambda(\mathbf x) - i e (A_\mu + \tfrac1e \partial_\mu \lambda(x)) ) e^{i \lambda(\mathbf x)} \psi(\mathbf x) \]
This can be written in terms of our original maps as
\[ \mathcal L'(\Lambda \mathbf x) = i \psi(\mathbf x)^\dag \sigma^\mu \Lambda^\nu_{\phantom\nu\mu} \partial_\nu \psi(\mathbf x) + i \psi(\mathbf x)^\dag \sigma^\mu \left[ i \Lambda^\nu_{\phantom\nu\mu} \partial_\nu \lambda(\mathbf x) - i e A'_\mu(\mathbf x) \right] \psi(\mathbf x) \]


If gauge invariance is to be preserved by each class of transformations (though the neat form taken by the equations of motion in the holonomic basis is generally not), then either
% the index on the vector potential $A_\mu$ must transform with the coordinates;
%
% if $A$ is a vector, 
% the components of the vector potential $A_\mu$ appearing in the Lagrangian must transform along with the coordinates.
% as part of the covariant derivative $\mathcal D_\mu = \partial_\mu - i e A_\mu$.
% transforming as $A_\mu \to A_\mu - \partial_\mu \lambda$, 
% the components of the vector potential of electromagnetism must transform with the coordinates to preserve gauge invariance.
%, even though it is presented as living in a four-dimensional tangent space.
% Since the gauge transformation takes the form $A_\mu \to A_\mu + \partial_\mu \lambda$ for some scalar function $\lambda(x)$, and invariance of the Lagrangian with respect to the choice of $\lambda(x)$ relies on commutation of the partial derivatives acting on $\lambda(x)$, the combination of derivative appearing in the Lagrangian must be antisymmetric $[\partial_\mu,\partial_\nu]\lambda(x)$ to be gauge invariant.
% Under a coordinate transformation
% This can be written in terms of our original maps and the transformation matrix $\Lambda$ as
% \[ \mathcal L'(\Lambda \mathbf x) = i \psi(\mathbf x)^\dag \sigma^\mu \Lambda^\nu_{\phantom\nu\mu} \partial_\nu \psi(\mathbf x) + i \psi(\mathbf x)^\dag \sigma^\mu \left[ i \Lambda^\nu_{\phantom\nu\mu} \partial_\nu \lambda(\mathbf x) - i e A'_\mu(\mathbf x) \right] \psi(\mathbf x) \]
% \[ (\partial_\mu - i e (A_\mu + \frac1e\lambda(\Lambda^{-1}\mathbf x) ) ) e^{i \lambda(\Lambda^{-1} \mathbf x)} \psi(\Lambda^{-1} \mathbf x) \]
% So $\partial_\mu \lambda$ must transform with the coordinates, as one would expect.
\begin{enumerate}
\item Gauge invariance is not preserved after a coordinate transformation alone, and both $A_\mu$ and $\partial_\mu \lambda$ transform with the basis of the tangent space.
\[ A_\mu \to A'_\mu = \Lambda^\nu_{\phantom\nu\mu} (A_\nu + \tfrac 1e \partial_\nu \lambda) \quad \text{(basis)} \] 
\item Gauge invariance is preserved, but 
% meant to cancel the derivative acting on the arbitrary phase of complex (e.g. spinor) fields.
\[ A_\mu \to A'_\mu = \begin{cases}
\Lambda^\nu_{\phantom\nu\mu} A_\nu + \tfrac 1e \partial_\mu \lambda & \text{(basis)} \\
A_\mu + \tfrac 1e \Lambda^\nu_{\phantom\nu\mu} \partial_\nu \lambda & \text{(coordinates)} \end{cases} \]
\item Gauge invariance is preserved, and the components of $A_\mu$ transform along with the coordinates.  Or, the components $A_\mu$ implicitly refer to the holonomic basis.
\[ A_\mu \to A'_\mu = \Lambda^\nu_{\phantom\nu\mu} (A_\nu + \tfrac 1e \partial_\nu \lambda) \quad \text{(coordinates)} \] 
\end{enumerate}
%
Option 1 is offensive on the grounds that we should be free to change how points in the space are labeled without unraveling the whole basis of electromagnetism.
Furthermore, the $\partial_\mu \lambda$ added to $A_\mu$ in the gauge transformation looks like it should transform like any other derivative of a scalar function.
Option 2 undermines the connection between $A_\mu$ and the gauge principle, since the gauge coupling term does not transform in the same way as the additive term involving $\partial_\mu \lambda$.
%
Option 3 suggests a picture of $A_\mu$ not as a geometric entity existing independently in a $3{+}1$-dimensional tangent space, but rather as something \emph{of} the coordinates.
% in need of a counterpart that does live in a tangent space with an independent basis and can carry energy.
Since the gauge field can be well understood as a connection allowing smooth differentiation between spinor spaces along curves in the manifold, it makes sense that has everything to do with the way events are labeled.
Then the covariant derivative transforms in a unified way under coordinate transformations.

We can get around this by using tetrad frame fields $e_a^{\phantom a \mu}$, and having the Greek index transform with the coordinates.
\[ D_\mu = \partial_\mu - i e e_\mu^{\phantom \mu a} A_a \qquad
 A_a \to A_a + \tfrac1e e_a^{\phantom a\nu} \partial_\nu \lambda \]
This saves the notion of a vector quantity $A$ as an abstract geometric object independent of reference frame.  But why is this more satisfying then simply asserting that the vector potential transforms with the coordinates?  Why must an unobservable quantity have a description-independent existence?

If $A_\mu$ transforms with the coordinates, then the standard second order kinetic term
$ F^{\mu\nu} F_{\mu\nu} $,
with $F_{\mu\nu} \equiv \partial_\mu A_\nu - \partial_\nu A_\mu$, is invariant under both coordinate and basis transformations performed separately -- in the sense that nothing transforms with an independently chosen basis for the tangent space.
% After all, the gauge theory accounts for extraneous degrees of freedom varying in space and time, and so perhaps should only be tied to how events are labeled.
%
% On the other hand, 
But there seems something off about a theory set in physical space that takes no account of a class of transformations affecting geometric objects bound therein.
We \emph{should} be free to deform the basis we adopt to describe the electromagnetic field while keeping the coordinates fixed, and to ask the theory directly what are the equations of motion in terms of those data.

%, and rather only depends on how the points of the space are labeled.
In the first order formulation of electromagnetism \cite{dirac}, one introduces variables for the electric and magnetic fields, taken {\it ab initio} to vary independently of $A_\mu$.  
 the first order Lagrangian takes the form
\begin{equation}
\mathcal L = F^{\mu\nu} \partial_\mu A_\nu - \tfrac18 F^{\mu\nu} F_{\mu\nu} \right]
\label{foem}
\end{equation}
% We do not want the Lagrangian to be invariant, since we want the equations of motion to reflect the fact that the basis with respect to which our data is defined is not aligned with the directions along which the coordinates increase.
% \begin{equation}
% \mathcal L = F^{ab} e_{a}^{\phantom a\mu} e_{b}^{\phantom b\nu} \partial_\mu A_\nu - \tfrac18 F^{ab} F_{ab} \right]
% \end{equation}
% In addition to the many simplications of using geometric algebra, 
% Varying with respect to the vector potential yields the inhomogeneous Maxwell equations, while varying with respect to $\mathcal F$ yields 
Assembling the Faraday tensor as a \emph{multivector} in the geometric algebra $\mathcal C \ell_3(\mathbb R)$ \cite{hest1,macd1}
%
\begin{equation} \mathcal F \equiv E^i \, \mathbf e_i + B^i \, \mathbf e_j \wedge \mathbf e_k \mapsto E^i \varsigma_i + \tfrac12 \epsilon_{ijk} B^i \varsigma_j \varsigma_k, \label{Fdef}  \end{equation}
where $\mathbf e_i$ are the vector elements of that algebra with matrix representations
\[ \varsigma^1 = \begin{pmatrix} \matzero & 1 & 0 & 0 \\ 1 & \matzero & 0 & 0 \\ 0 & 0 & \matzero & -i \\ 0 & 0 & i & \matzero \end{pmatrix}} \quad
\varsigma^2 = \begin{pmatrix} \matzero & 0 & 1 & 0 \\ 0 & \matzero & 0 & i \\ 1 & 0 & \matzero & 0 \\ 0 & -i & 0 & \matzero \end{pmatrix} \quad
\varsigma^3 = \begin{pmatrix} \matzero & 0 & 0 & 1 \\ 0 & \matzero & -i & 0 \\ 0 & i & \matzero & 0 \\ 1 & 0 & 0 & \matzero \end{pmatrix} \]
% are matrix representations of vector elements of that algebra, 
satisfying $\varsigma^1 \varsigma^2 = i \varsigma^3$ and $-i \varsigma^1 \varsigma^2 \varsigma^3 = I_4 \equiv \varsigma^0$, this can be put into a form resembling the Dirac equation:
\[ \mathcal L = \mathcal F \, \Pi^{\mu\nu} \partial_\mu A_\nu - \tfrac18 \mathcal F^2 + \text{h.c.} \]
Here, $\Pi^{\mu\nu}$ are a set of 16 constant elements with $4 \times 4$ matrix representations  $(\Pi^{\mu\nu})^{ab} = \eta^{\mu a} \delta^{\nu b} $; like the gamma matrices in the Dirac equation, the Greek indicies on $\Pi^{\mu\nu}$ merely label elements, and do not transform with the coordinates or basis.

What are taken as the definitions of $\mathbf E$ and $\mathbf B$ in terms of the exterior derivative of $A$ fall out of the Euler-Lagrange equations as six non-dynamical constraints.
Since no time derivatives of $E_i$, $B_i$ appear in the Lagrangian, they are in effect Lagrange multipliers, and the equations obtained by requiring the variation of the action with respect to them to vanish must be treated as identities (eventually, not subject to quantum uncertainty).  When the components of $\mathbf E$ and $\mathbf B$ refer to the holonomic basis
\[ \fdx{S}{E_i} = E_i - (\partial_0 A_i - \partial_i A_0) \equiv 0 \qquad \fdx{S}{B_i} = -B_i + (\partial_j A_k - \partial_k A_j) \equiv 0 \qquad \fdx{S}{A_0} = \partial_i E^i \]
After integrating out the non-dynamical degrees of freedom, we are left with three dynamical degrees of freedom in $A_i$ ($A_0$ is also a Lagrange multiplier).

While in most respects a trivial reframing, this formulation allows us to sidestep the apparent conflict between the second order theory and the intuition stated above.  
Let new coordinates $\bar x^\mu$ be related to the old as $\bar x^\mu = \Lambda^\mu_{\phantom\mu\nu} x^{\nu}$, and let \[S = \exp \left({\frac12\theta_i [\varsigma^j, \varsigma^k] + \frac12 w_i \varsigma^i}\right)\] operate on elements of the geometric algebra to enact a proper basis transformation.
If the object $\mathcal F$ -- which plays no direct role in the gauge covariant derivative -- transforms with the basis of the tangent space spanned by multivectors, 
% Changing the coordinates or basis alone keeps the coupling between $\mathcal F$ and its sources invariant, but changes the definition of $\mathcal F$ in terms of $A_\mu$.
%\footnote{This move also democratizes spin. Since the field theory must be cast in terms of linear operators acting on state vectors, the derivative can be taken as acting to the right or, in a subtly modified way, to the left.  A steady time-varying rotation of the coordinates \emph{or} the basis of the multivector tangent space results in the same additional term in the Lagrangian depending on $\dx\theta/\dx t$.}.
then \eqref{foem} transforms as
\begin{equation} \mathcal L \to \begin{cases} S \mathcal F(\mathbf x) S^{-1}  \Pi^{\mu\nu} \partial_\mu A_\nu(\mathbf x) - \tfrac18 {(S \mathcal F(\mathbf x) S^{-1})^2} & \text{(basis)} \\ 
\mathcal F(\Lambda^{-1} \mathbf x) \, \Pi^{\mu\nu} \partial_{\mu} \Lambda^{\rho}_{\phantom{\nu}\nu} A_{\rho}(\Lambda^{-1}\mathbf x) - \tfrac18 \mathcal F(\Lambda^{-1}\mathbf x)^2 & \text{(coordinates)} \end{cases} \end{equation}
%
% (Under the trace, $(S \mathcal F S^{-1})^2$ is equivalent to $\mathcal F^2$ due to the cyclic property.)
with an overall trace of the Hermitian part implied.
(Since the variables making up $\mathcal F$ are Lagrange multipliers, we can have them transform in any we want.)
In this form, the equations of motion still describe gauge-invariant electromagnetism after a transformation of the coordinates or the basis for $\mathcal F$, but are only fully invariant under complementary transformations acted together.
\[ \mathcal L = e^{a\mu} (\partial_a A_b - \partial_b A_a) e^{b\nu} (\partial_\mu A_\nu - \partial_\nu A_\mu) \]
where $e^a_{\phantom a \mu}$ are the tetrad fields.

% -- befitting for a vector field theory.
% The Lagrangian does not track some invariant measure of the spatial and temporal dependence of $\psi$, as it would for a scalar field.  Rather, it tracks the derivative of the components of $\psi$ for which $\psi\psi^\dag$ is oriented along the direction in which $x^\mu$ increases.  So under a true coordinate transformation, we must change the reference elements $\varsigma^\mu$ that we use to query the orientation of $\psi\psi^\dag$.
% % The basis of $\partial = \varsigma^\mu \partial_\mu$ transforms as a four-covector, $\varsigma^\mu \to S^\dag \varsigma^\mu S$, and the components transform as a four-vector, $\partial_\mu \to \Lambda_\mu^{\phantom\mu\nu} \partial_\nu$, such that the overall vector is unchanged: $\partial \to S^\dag \varsigma^\mu S \Lambda_\mu^{\phantom\mu\nu} \partial_\nu = \varsigma^\mu\partial_\mu$.  
% \[ \mathcal L \to i \psi(x^{\mu'})^\dag (S^\dag \varsigma^\mu S) \partial_\mu \psi(x^{\mu'}) 
% = \mathcal L \]
On the other hand, the gauge theory exists to account for extraneous nonphysical degrees of freedom varying in space and time, and so perhaps should only be tied to how events are labeled -- leaving the basis choice for $\mathbf E$ and $\mathbf B$ to be established in the terms of the Lagrangian describing the measuring apparatus.
% \[ \mathcal L = \bra\Psi F^{\mu\nu} \partial_\mu A_\nu - \tfrac14 F^{\mu\nu} F_{\mu\nu} \ket\Psi \]
% The above describes a passive transformation; we have not really done anything to the field, simply relabeled points on the space in which it lives, and realigned our reference grid of basis vectors to align with the new coordinates.  There is of course an active transformation in which the field at each point changes.

%  If we insist on changing the components of $\partial$ without changing the basis of that multivector,
% then the leftover basis transformation must be compensated on each side by the basis transformations of $\psi$ and $\psi^\dag$.  
% Or, equivalently, if we change the mapping between $\partial_\mu$ and the argument of the field components $\psi_A(x^\mu)$, say by transforming $\psi_A(x^\mu) \to \psi_A(\Lambda^\mu_{\phantom\mu\nu} x^\nu)$, then we must change the basis of $\psi$ as well to leave the Lagrangian invariant.
% However, \eqref{eq:galagrangian} alone does not fully dictate the transformation law that the basis and components of $\psi$ obey.

% If we allow the basis or components of $\psi$ to transform such that $\psi \to S\psi$, where $S$ defines a basis rotation that may depend on $x^\mu$, we obtain the above transformation up to a term dependent on $\partial'_\mu S(\mathbf x) = \partial_\mu S(\mathbf x') = \Lambda_\mu^{\phantom\mu\nu} \partial_\nu S(\mathbf x)$.  Subtracting that term, we have
% \begin{equation} \mathcal L \to i (S\psi)^\dag \varsigma^\mu \partial'_\mu (S \psi) - i (S\psi)^\dag \varsigma^\mu (\partial'_\mu S S^{-1}) (S \psi) = i \psi^\dag \varsigma^\mu \partial_\mu \psi \label{eq:spinorcovder} \end{equation}
% We know that the intrinsic angular momentum should be $\tfrac12$, so we need to make a distinction between coordinate transformations and basis transformations, each of which contribute a term of magnitude $\tfrac12 \dot\theta \psi^\dag \psi$ but of opposite sign when a rotation takes place about $\langle\psi\psi^\dag\rangle_1$ by an angle $\theta(t)$, which cancel out when acted together.
% This way, the Lagrangian changes by $\tfrac12 \dot\theta \psi^\dag\psi$ whether we rotate the basis of the tangent space at every event or mix the components of the derivative to reflect a time-dependent coordinate transformation.
% %
% % Let us say that the first term comes about from the product rule applied to the transformed basis, and the second term comes from a covariant derivative that transforms with the coordinates.
% \[ \mathcal L \to \begin{cases}
% i (S\psi)^\dag \varsigma^\mu \partial_\mu (S \psi) & \text{(basis)} \\
% i \psi^\dag \varsigma^\mu \Lambda_{\mu}^{\phantom\mu\nu} (\partial_\nu - \partial_\nu S S^{-1}) \psi & \text{(coordinate)}
% \end{cases}
%  \]
% %
% % So under this partial transformation, we can treat $\psi$ as transforming into $S \psi$, as long as we account for the covariant derivative associated with a local dependence of $S$.
% %
% % We obtain the second term in the above coordinate transformation by replacing the partial derivative $\partial_\mu$ with a coordinate-covariant derivative $\nabla_\mu$, 
% % \[ \mathcal \nabla_\mu \psi \equiv \partial_\mu \psi + \omega_\mu \psi \to \Lambda_\mu^{\phantom\mu\nu} (S \partial_\nu (S^{-1} \psi) + \omega_\nu \psi) , \]
% % introducing a spin connection term $i\psi^\dag\varsigma^\mu\omega_\mu\psi$, which becomes  
% % \[ \omega_\mu \to \begin{cases}
% % S \omega_\mu S^{-1} & \text{(basis transformation)} \\
% % \Lambda_\mu^{\phantom\mu\nu} (\omega_\nu - \partial_\nu S S^{-1}) & \text{(coordinate transformation)} 
% % \end{cases} \]

% \chapter{First Order}

% The equations of motion should be covariant under coordinate or basis transformations, but the two terms transform differently (the second is invariant under both).  If we include a field that transforms as a 4-vector under both transformations, then both terms can transform in the same way.

% \begin{center}
% \noindent\rule{8cm}{0.4pt}
% \end{center}
% \vspace{.2cm}

\subsection{$SU(2)$}

We can arrive at the kinetic Lagrangian for the $SU(2)$ gauge field not by asserting overall gauge invariance of the Lagrangian, but only asserting that the quantum field theory be algebraically consistent.
\[ \mathcal L = \Tr \left[  G^{\mu\nu} \partial_\mu  W_\nu - \tfrac18  G^{\mu\nu}  G_{\mu\nu} \right] \]
where $G^{\mu\nu}$ are Lagrange multipliers.
% \[ G_{\mu\nu} = \partial_\mu W_\nu - \partial_\nu W_\mu \]
% \[ G_{\mu\nu} = \partial_\mu (U W_\nu U^\dag - i U \partial_\nu U^\dag) - \partial_\nu (U W_\mu U^\dag - i U \partial_\mu U^\dag) \]
% \[ G_{\mu\nu} = \partial_\mu (U W_\nu U^\dag) - \partial_\nu (U W_\mu U^\dag) - i \partial_\mu U \partial_\nu U^\dag + i \partial_\nu U \partial_\mu U^\dag \]
Under a gauge transformation, we have
\[ \mathcal L = \Tr \left[ G^{\mu\nu} \partial_\mu (U \mathcal W_\nu U^\dag - i U \partial_\nu U^\dag) - \tfrac18 G^{\mu\nu} G_{\mu\nu} \right] \]
If $ G^{\mu\nu}$ is anti-symmetric in its Greek indices, then the non-covariant term coming from the transformation of $ W_\nu$ -- which involves the second derivative of $S$ -- vanishes.
Since $G^{\mu\nu}$ are Lagrange multipliers that will be integrated out in the end, we are free to have them transform however we like under gauge transformations, so let us say $\mathcal G^{\mu\nu} \to U \mathcal G^{\mu\nu} U^\dag$.
If the gauge transformation is homogeneous in space and time, we can use the cyclic property of the partial trace to cancel 
\[ \mathcal L = \Tr \left[ U  G^{\mu\nu} U^\dag U \partial_\mu  W_\nu U^\dag - \tfrac18 U  G^{\mu\nu}  G_{\mu\nu} U^\dag \right] = \Tr \left[  G^{\mu\nu} \partial_\mu  W_\nu - \tfrac18  G^{\mu\nu}  G_{\mu\nu} \right] \]
If the transformation is not uniform, then we get operators $U$ and $U^\dag$ acting directly on the quantum state $\ket\Psi$.  
\[ \mathcal L = \Tr \left[ \bra{\Psi} \left( U  G^{\mu\nu} U^\dag \partial_\mu (U  W_\nu U^\dag + i ( \partial_\nu U) U^\dag) - \tfrac18 U  G^{\mu\nu}  G_{\mu\nu} U^\dag \right) \ket{\Psi} \right] \] 
\[ \mathcal L = \Tr \left[ \bra{\Psi} \left( U  G^{\mu\nu} U^\dag \partial_\mu (U  W_\nu U^\dag ) - \frac18  G^{\mu\nu}  G_{\mu\nu} \right) \ket{\Psi} \right] \]
But the state vector $\ket\Psi$ does not contain a copy of the gauge space on which $U$ is to act, and $U$ does not constitute a map from the state space to $SU(2)$, as does the field operator $\hat{ W_\mu}$.
Furthermore, it is the gauge component of $\hat { W_\mu} \ket{\Psi}$ that transforms like $U ({}\cdot{}) U^{\dag}$, but the column index of the field operator itself must run over the space of quantum states, and cannot receive multiplication by $U^{\dag}$ from the right; so $\hat{ W}_\mu \to U \hat{ W}_\mu U^\dag$ does not even make sense mathematically.
The Lagrangian must be constructed such that all \emph{outer} transformation operators that do not act explicitly on and only on the space of states can be omitted without consequence.

Rearranging the above expression to isolate the residual outer operators yields
\[ \mathcal L = \Tr \left[  G^{\mu\nu} U^\dag \partial_\mu (U  W_\nu ) +  G^{\mu\nu} ( W_\nu ) (\partial_\mu U^\dag) U - \tfrac18  G^{\mu\nu}  G_{\mu\nu} \right] \]
%
% We can eliminate the second term by including another term in the Lagrangian coupling to $ W_\mu$.
In order to construct a Lagrangian that can be transformed by inner linear operations alone, we can add a coupling term with $ W_\mu$ multiplying from the right
\[ \mathcal L = \Tr \left[  G^{\mu\nu} \partial_\mu  W_\nu - i  G^{\mu\nu}  W_\nu  W_\mu - \tfrac14 G^{\mu\nu} G_{\mu\nu} \right] \]
The non-covariant term coming from the transformation of $W_\nu$ cancels the term above involving the outer factor of $\partial_\mu U$, serving the same function for which it was originally intended in the fermionic Lagrangian.
\[ \mathcal L = \Tr \left[  G^{\mu\nu} U^\dag \partial_\mu (U  W_\nu) - i  G^{\mu\nu} ( W_\nu + i U^\dag \partial_\nu U)  W_\mu + \cdots \right] \]
If $ G^{\mu\nu}$ is anti-symmetric in its Greek indices, then the non-covariant term coming from the transformation of $ W_\nu$ -- which involves the second derivative of $S$ -- vanishes. 
% But this Lagrangian has the same problem discussed above -- hanging outer transformation operators that cause problems when we promote fields to field operators.
% \[  L = \Tr \left[  G^{\mu\nu} U^\dag \partial_\mu (U  W_\nu) + U  G^{\mu\nu} U^{\dag}  W_\nu \partial_\mu U^{\dag} - \tfrac18  G^{\mu\nu}  G_{\mu\nu} \right] \]
% In order to construct a Lagrangian that can be transformed by inner linear operations alone, we can perform the same trick of adding a coupling term to $ W_\mu$
% \[ \mathcal L = \Tr \left[ \mathcal G^{\mu\nu} \partial_\mu \mathcal W_\nu - i \mathcal G^{\mu\nu} \mathcal W_\nu \mathcal W_\mu \right] \]
% This not only eliminates the outer transformation operators, but makes the kinetic Lagrangian invariant under basis transformations.
% \[ \mathcal L = \Tr \left[ \mathcal G^{\mu\nu} S^{-1} \partial_\mu (S \mathcal W_\nu + i \partial_\nu S) - i \mathcal G^{\mu\nu} (\mathcal W_\nu + i S^{-1} \partial_\nu S) \mathcal W_\mu + \cdots \right] \]
The remaining new terms after the transformation are
\[ \delta \mathcal L = \Tr \left[ \mathcal G^{\mu\nu} (U^{\dag} \partial_\mu U) \mathcal W_\nu + \mathcal G^{\mu\nu} ( U^{\dag} \partial_\nu U) \mathcal W_\mu + \cdots \right] \]
which also vanish due to anti-symmetry of $\mathcal G^{\mu\nu}$.
\begin{equation} \mathcal L = \Tr \left[ \mathcal G^{\mu\nu} \partial_\mu \mathcal W_\nu - i \mathcal G^{\mu\nu} \mathcal W_\nu \mathcal W_\mu - \tfrac1{8} \mathcal G^{\mu\nu} \mathcal G_{\mu\nu} + \text{h.c.} \right] \end{equation}
So in requiring only that the outer gauge transformation operators cancel out, we have by accident made the whole kinetic Lagrangian invariant under gauge transformations!

The Euler-Lagrange equation when varying with respect to $G^{\mu\nu}$ gives
\[ G_{\mu\nu} \equiv \partial_\mu W_\nu - \partial_\nu W_\mu + ig ( W_\mu W_\nu - W_\nu W_\mu) \]
which must be treated as a constraint since no time derivatives of $G^{\mu\nu}$ appear in the Lagrangian.
Integrating $G^{\mu\nu}$ out of the Lagrangian yields the standard form in terms of only $W_\mu$.

\subsection{subsection}

% \[ \mathcal F \equiv E_i \varsigma^i + B_i \varsigma^j \varsigma^k \]
If $A_\mu$ and $\mathcal F$ represent the same physical degrees of freedom,
%-- due to the extra Euler-Lagrange equations amounting to constraints -- 
what is the role for $A_\mu$ in the absence of source terms?
Can we write down a Lagrangian involving only $\mathcal F$ that describes the same free physics, as we can write down a theory involving only $A_\mu$?
% (The short answer: 'no.')
The short answer is `no,' but thinking carefully through a few of the reasons why that is the case in the context of the above discussion is, in our view, worthwhile.

Assembling the Faraday tensor as a \emph{multivector} in the geometric algebra $\mathcal C \ell_3(\mathbb R)$ \cite{hest1,macd1}
%
\begin{equation} \mathcal F \equiv E^i \, \mathbf e_i + B^i \, \mathbf e_j \wedge \mathbf e_k \mapsto E^i \varsigma_i + \tfrac12 \epsilon_{ijk} B^i \varsigma_j \varsigma_k, \label{Fdef}  \end{equation}
where $\mathbf e_i$ are the vector elements of that algebra with matrix representations
\[ \varsigma^1 = \begin{pmatrix} \matzero & 1 & 0 & 0 \\ 1 & \matzero & 0 & 0 \\ 0 & 0 & \matzero & -i \\ 0 & 0 & i & \matzero \end{pmatrix}} \quad
\varsigma^2 = \begin{pmatrix} \matzero & 0 & 1 & 0 \\ 0 & \matzero & 0 & i \\ 1 & 0 & \matzero & 0 \\ 0 & -i & 0 & \matzero \end{pmatrix} \quad
\varsigma^3 = \begin{pmatrix} \matzero & 0 & 0 & 1 \\ 0 & \matzero & -i & 0 \\ 0 & i & \matzero & 0 \\ 1 & 0 & 0 & \matzero \end{pmatrix} \]
% are matrix representations of vector elements of that algebra, 
satisfying $\varsigma^1 \varsigma^2 = i \varsigma^3$ and $-i \varsigma^1 \varsigma^2 \varsigma^3 = I_4 \equiv \varsigma^0$,
consider the first order Lagrangian
\begin{equation} \mathcal L = \mathcal F^\dag \varsigma^1 \varsigma^2 \varsigma^3 \partial_0 \mathcal F - \tfrac12 \epsilon_{ijk} \mathcal F^\dag \varsigma^i \varsigma^j \partial_k \mathcal F \quad \text{(implied trace)} \label{foga} \end{equation}
The corresponding Euler-Lagrange equations are, perhaps unsurprisingly, six of Maxwell's equations in the absence of sources when varying with respect to the vector and bivector degrees of freedom represented in \eqref{Fdef}.
% If we take $\mathcal F$ to be a general element of the geometric algebra in three dimensions, then there are also scalar and pseudo-scalar degrees of freedom.
% Varying with respect to scalar and pseudo-scalar degrees of freedom -- and then fixing them to vanish -- gives the remaining two.
%
Why then do we not encounter \eqref{foga} in the Standard Model, characterizing elementary fields with integer spin?
The Lagrangian is not invariant under boosts, where the transformation operator satisfies $S^\dag = S$,
\begin{equation} \mathcal L \to i (S^{-1})^\dag \mathcal F^\dag(\Lambda^{-1} \mathbf x) S^\dag \varsigma^\mu \partial_{\mu} (S \mathcal F(\Lambda^{-1} \mathbf x) S^{-1}) \label{foga_trans} \end{equation}
% \begin{equation} \mathcal L \to (S^{-1})^\dag \mathcal F^\dag S^\dag \left[ i (\Lambda^{-1})_0^{\phantom0\mu} - i \varsigma^k (\Lambda^{-1})_k^{\phantom k \mu} \right] \partial_{\mu} (S \mathcal F S^{-1}) \label{foga_trans} \end{equation}
but it is under uniform rotations $((S^{-1})^\dag = S)$. 

Solutions to the equations of motion are the same in all inertial reference frames if and only if we include dynamical scalar and pseudo-scalar degrees of freedom in $\mathcal F$, departing from Maxwell.  
\begin{equation} \mathcal F \equiv \phi + E^i \, \mathbf e_i + B^i \, \mathbf e_j  \mathbf e_k + \chi \, \mathbf e_1  \mathbf e_2  \mathbf e_3 \mapsto (\phi + i \chi)\varsigma_0 + (E^j + i B^j ) \varsigma_j, \label{Fdef2} \end{equation}
After a boost, varying with respect to the original 8 degrees of freedom yields 4 pairs of equations taking the form
\[ \fdx{S'}{A} = \fdx{S}{A} \cosh w + \fdx{S}{B} \sinh w \qquad \fdx{S'}{B} = \fdx{S}{B} \cosh w + \fdx{S}{A} \sinh w \]
Since $\cosh w \neq \sinh w$ for all $w \in \mathbb R$, requiring that the action be stationary results in the same classical equations of motion for fields before and after the transformation.
\[ \fdx{S'}{A} = \fdx{S'}{B} = 0 \implies \fdx{S}{A} = \fdx{S}{B} = 0 \]
This must be the case, since rotations and boosts do not commute, and the Lagrangian is invariant under homogeneous basis and coordinate rotations.
But we care about more than just locations of stationary points in configuration space.  The quantities $\delta S/\delta A$ also tell us about probabilities for non-classical configurations, and should be the same in different equivalent representations of the system.
% \begin{equation} \mathcal L = i \mathcal F^\dag \varsigma^\mu \partial_\mu \mathcal F \end{equation}
% \begin{equation} \mathcal L = i \varsigma^\mu \mathcal F^\dag \varsigma^\nu \epsilon_\mu \partial_\nu \mathcal F \to i S \varsigma^\mu S^\dag S^{-\dag} \mathcal F^\dag S^\dag \varsigma^\nu \epsilon_\mu \partial'_\nu (S \mathcal F S^{-1}) \end{equation}
% % A general Lorentz transformation then takes the form
% % \begin{equation} \mathcal L = i S \varsigma^\mu S^\dag S^{-\dag} \mathcal F^\dag S^\dag \varsigma^\nu \epsilon_\mu \partial'_\nu (S \mathcal F S^{-1}) \end{equation}
% If the transformation $S$ is homogeneous, then with the cyclic property of the trace we have
% \begin{equation} \mathcal L = i \varsigma^\mu \mathcal F^\dag S^\dag \varsigma^\nu S \epsilon_\mu \partial'_\nu \mathcal F \end{equation}

Because the Hamiltonian is not bounded from below, the creation and annihilation operators would have to anti-commute.
Also the Lagrangian is invariant with respect to a global phase change, and so this field should couple to a $U(1)$ gauge field.

For now, let us fix the time-space cut and consider how a quantum field theory governed by \eqref{foga} (or at least the positive frequency sector) behaves under 
% arbitrary transformations among the spatial coordinates and 
local rotations of the tangent basis.  
% However, after the transformation there is a term with $\partial_\nu S^\dag$ in the rightmost position, and $S$ in the leftmost.
For this, we promote $\mathcal F$ to a field operator $\hat{\mathcal F}$, which acts on the state vector $\ket{\varPsi}$.
% \[ \hat{\mathcal F}(x) = \sum_s \int \frac{\dx^4 k}{(2\pi)^4} \, \Theta(k_0) u_s \left( e^{-i k x} \hat b_{k,s} + e^{ikx} \hat c_{k,s}^\dag \right) \sqrt{2 k_0} \]
\[ \hat{\mathcal F}(x) = \sum_s \int \frac{\dx^3 k}{(2\pi)^3 (2 k_0)} \, u_s \left( e^{-i k x} \hat b_{k,s} + e^{ikx} \hat c_{k,s}^\dag \right) \sqrt{2 k_0} \]
Here $u_s$ is not a function of $k$, and $s$ goes over all of the degrees of freedom of $\mathcal F$.

A quantum field theory must be formulated as a sequence of linear operators modifying state vectors, and any transformation of the coordinates or tangent basis must conform to this representation.
We can affect a coordinate transformation by acting with a unitary operator and its inverse upon the creation and annihilation operators, which in turn act on vectors in the space of quantum states.
\[ U_\Lambda \hat b_{k,s} U_\Lambda^{-1} \sqrt{2 k_0} = \hat b_{k\Lambda^{-1},s} \sqrt{2 (k \Lambda^{-1})_0} \]
\begin{align*}
U_\Lambda \hat{\mathcal F}(x) U_\Lambda^{-1} &= \sum_s \int \frac{\dx^3 k}{(2\pi)^3 (2 k_0)} \, u_s \left( e^{-i k x} U_\Lambda \hat b_{k,s} U_\Lambda^{-1} + e^{ikx} U_\Lambda \hat c_{k,s}^\dag U_\Lambda^{-1} \right) \sqrt{2 k_0} \\
\[ U_\Lambda \hat{\mathcal F}(x) U_\Lambda^{-1} &= \sum_s \int \frac{\dx^3 k}{(2\pi)^3 (2 k_0)} \, u_s \left( e^{-i k x} \hat b_{k\Lambda,s} + e^{ikx} \hat c_{k\Lambda,s}^\dag \right) \sqrt{2 (k\Lambda)_0} \\
\[ U_\Lambda \hat{\mathcal F}(x) U_\Lambda^{-1} &= \sum_s \int \frac{\dx^3 k'}{(2\pi)^3 (2 k'_0)} \, u_s \left( e^{-i k' \Lambda x} \hat b_{k',s} + e^{ik' \Lambda x} \hat c_{k',s}^\dag \right) \sqrt{2 k_0'} \end{align*}
% 
But objects living in the tangent space must, we assert, be represented in terms of geometric algebra, transforming by means of multiplication on both sides by elements of the appropriate cover of the Lorentz group.  
So we should be able to either transform the index $s$ on the ladder operators or act with the operator $S$ on the geometric algebra; the reults must be equivalent.
%
% A transformation of the coordinates or tangent basis is not exempt, but must too be cast as the action of operators on state vectors.
%
\[ \hat{\mathcal F}(x) \to \sum_s \int \frac{\dx^3 k}{(2\pi)^3 \sqrt{2 k_0}} \begin{cases}  S u_s S^{-1} \left( e^{-i k x} \hat b_{k,s} + e^{ikx} \hat c_{k,s}^\dag \right) \\ u_s \left( e^{-i k x} \hat b_{k,s'} + e^{ikx} \hat c_{k,s'}^\dag \right) \end{cases} \]
When the transformation is homogeneous in space and time, we can use the cyclic property of the partial trace over the geometric algebra implied in \eqref{foga}, to cancel the left-most $(S^{-1})^\dag = S$ and the right-most $S^{-1}$ 
% in from the basis transformed version \eqref{foga_trans}
\begin{equation} \expv{\mathcal L} \to 
\bra{\varPsi} S \hat{\mathcal F}^\dag S^\dag (i\varsigma^\mu) \partial_\mu S \hat{\mathcal F} S^{-1} \ket{\varPsi} \overset{\partial S = 0}{- \!\!\! \longrightarrow} 
i \bra{\varPsi} \hat{\mathcal F}^\dag S^\dag \varsigma^\mu S \partial_\mu \hat{\mathcal F} \ket{\varPsi} \end{equation}
leaving only field operators at the edges mapping the state to a tensor product space that includes a copy of the multivector tangent space. 

If the basis transformation is not uniform, then we get $S$ acting on $\bra{\varPsi}$ and $\partial_\mu S^{-1}$ acting on $\ket{\varPsi}$.
% \[ \mathcal L \to 
% \bra{\Psi} i \hat{\mathcal F}^\dag S^\dag \varsigma^\mu \partial_\mu S \hat{\mathcal F} \ket{\Psi} + 
% \bra{\Psi} i S \hat{\mathcal F}^\dag S^\dag \varsigma^\mu S \hat{\mathcal F} (\partial_\mu S^\dag) \ket{\Psi} \]
% which is unacceptable for the reasons stated above.  
%
But $\ket{\varPsi}$ does not contain a copy of the tangent space on which $S$ is to act, and the operator $S$ does not constitute a map from the state space to the tangent space, as does the field operator $\hat{\mathcal F}$.
Furthermore, it is the geometric component of $\hat {\mathcal F} \ket{\Psi}$ that transforms like $S \mathcal F S^{-1}$, but the column index of the field operator itself must run over the space of quantum states, and cannot receive multiplication by $S^{-1}$ from the right.
To be consistent with quantum theory, a global basis transformation cannot {require} multiplication by $S^{-1}$ from the right on the right-most field operator $\hat{\mathcal F}$, between the latter and the quantum state $\ket{\varPsi}$;
% \vspace{.3cm}
%
% \begin{description} \it
the Lagrangian must be constructed such that {all} \emph{outer} transformation operators can be omitted without consequence.
% \end{description}
This algebraic criterion alone rules out \eqref{foga} as a theory of integer spin fields.

This can be resolved of course by substituting for $\hat{\mathcal F}$ a spinor field $\hat\psi$ transforming explicitly as $\hat S \hat \psi \ket{\Psi}$, where $\hat S$ transforms elements of the geometric algebra while acting as the identity on the state vector.
In order to accommodate a kinetic term resembling \eqref{foga} for a true multivector field, one would have to introduce a vector field that transforms non-covariantly under basis rotations:
%, to cancel the derivative of $S^{\dag}$ acting on $\hat{\mathcal F}$ from the right.
% This field, which we denote $\mathcal W_\mu$, transforms under coordinate \emph{and} basis rotations:
\begin{equation} \mathcal W_\mu \to \begin{cases}
S \mathcal W_\mu S^{-1} - i S \partial_\mu S^{-1} & \text{(basis)} \\
% under basis transformations and 
\Lambda^\nu_{\phantom\nu\mu} \mathcal W_{\nu} & \text{(coordinates)} 
\end{cases} \label{Wdef} \end{equation}
Using \eqref{Wdef} and the (distinct) spin connection transforming as 
$ \omega_\mu \to \Lambda^\nu_{\phantom\nu\mu} (\omega_\nu - S_{\Lambda}^{-1} \partial_\nu S_{\Lambda} ) $ % \quad \text{(coordinate)}\]
with the coordinates and $ \omega_\mu \to S \omega_\mu S^{-1}$ with the basis, 
there are two available modifications to \eqref{foga} that resolve the issue and manifest the desired symmetry between coordinate and basis transformations:
\begin{equation}
\mathcal L = i\mathcal F^\dag \varsigma^\mu \partial_\mu \mathcal F + \begin{cases} \mathcal F^\dag \varsigma^\mu \mathcal F \mathcal W_\mu + i\mathcal F^\dag \varsigma^\mu \omega_\mu \mathcal F & (1)\\
 \mathcal F^\dag \varsigma^\mu \mathcal F \mathcal W_\mu - 2 \mathcal F^\dag \varsigma^\mu \mathcal W_\mu \mathcal F - i\mathcal F^\dag \varsigma^\mu \omega_\mu \mathcal F & (2)
 \end{cases}
 \label{blah}
\end{equation}
% (with an overall trace and hermitian part implied).  
Using $S \partial_\mu S^\dag = - S^\dag \partial_\mu S$,
under a local rotation of the tangent basis we have
% with $\mathcal F \to S\mathcal F S^\dag$
\begin{equation} \mathcal L \to \begin{cases} i\mathcal F^\dag \varsigma^{\mu'} S^\dag \partial_{\mu} (S \mathcal F) + \mathcal F^\dag \varsigma^{\mu'} \mathcal F \mathcal W_\mu + i\mathcal F^\dag \varsigma^{\mu'} \omega_\mu \mathcal F \\
 i\mathcal F^\dag \varsigma^{\mu'} S \partial_\mu (S^\dag \mathcal F) + \mathcal F^\dag \varsigma^{\mu'} \mathcal F \mathcal W_\mu - 2 \mathcal F^\dag \varsigma^{\mu'} \mathcal W_\mu \mathcal F - i\mathcal F^\dag \varsigma^{\mu'} \omega_\mu \mathcal F
 \end{cases} \end{equation}
where $\varsigma^{\mu'} \equiv S^\dag \varsigma^{\mu} S$.  
% Under the complementary coordinate transformation
% \[\mathcal L \to \begin{cases} i\mathcal F^\dag \varsigma^{\mu} S \partial_{\mu'} (S^\dag \mathcal F) + \mathcal F^\dag \varsigma^{\mu} \mathcal F \mathcal W_{\mu'} + i\mathcal F^\dag \varsigma^{\mu} S \omega_{\mu'} S^\dag \mathcal F \\
%  i\mathcal F^\dag \varsigma^{\mu} S^\dag \partial_{\mu'} (S \mathcal F) + \mathcal F^\dag \varsigma^{\mu} \mathcal F \mathcal W_{\mu'} - 2 \mathcal F^\dag \varsigma^{\mu} \mathcal W_{\mu'} \mathcal F - i\mathcal F^\dag \varsigma^{\mu} S \omega_{\mu'} S^\dag \mathcal F \end{cases} \]
Under complementary basis and coordinate rotations acted together, the Lagrangian is of course invariant.
% up to terms depending on $\partial_\mu\theta$.

% \chapter{What is angular momentum?}
% We intuitively think of angular momentum as made up of well defined contributions from particular entities (objects, fields, etc.), relating to how each transforms under rotations in isolation from the rest of the system.
% But the notion of angular momentum derived from Noether's theorem is more consistent with rotations in a global sense: how does the whole system respond to a steady rotation of the tangent basis or coordinates?


If we identify rotations of the orientation angle invoked in Noether's theorem with global transformations of the coordinates\footnote{apart from the spin connection's non-covariant additive term} and the tangent bases to which the components of all fields in the system refer, then $\mathcal F$ ``no longer'' represents an integer spin field.  
Multivector fields governed by the two Lagrangians in \eqref{blah} \emph{effectively} transform as left- and right-chiral Weyl spinor doublets,
owing to the non-covariant term coming from \eqref{Wdef} cancelling the other ``half'' of the kinetic term's intrinsic dependence on $\dx\theta/\dx t$. 

Note that we {have not} introduced a second copy of the reference basis for the multivector tangent space with opposite orientation (e.g.\ $\bar\varsigma^1\bar\varsigma^2 = -i \bar\varsigma^3$) in order to accommodate two chiralities;
it is the form of the Lagrangian -- the nominal coupling to the non-covariant field $\mathcal W_\mu$ -- that \emph{determines} chirality.

% This scheme opens up the possibility that the spin angular momentum associated with a field's excitations is not fully dictated by how the geometric object underlying the field transforms.  Excitations of the same geometric object (multivector) can have spin-0, $\tfrac12$, or 1 depending on the Lagrangian, as long as the constraints are satisfied.  
% The general form allowed by the above considerations and consistency with quantization of angular momentum is
% \[ i\hat{\mathcal F}^\dag \varsigma^\mu \partial_\mu \hat{\mathcal F} + \hat{\mathcal F}^\dag \varsigma^\mu \hat{\mathcal F} \hat{\mathcal W_\mu} - n \hat{\mathcal F}^\dag \varsigma^\mu \hat{\mathcal W_\mu} \hat{\mathcal F} \]
% where the integer $n$ can take values 0 or 2.
% For $n = 0$, we get the left-chiral field discussed above.  
% % With $n=1$, both additional terms coming from $\partial_\nu$ acting on $S\mathcal F S^\dag$ are cancelled, so the spin angular momentum is zero, and we have a multiplet of scalar fields.  
% For $n=2$, the spin angular momentum of the $n=0$ case is negated, resulting in a half-integer spin field of the opposite chirality.
% %
% % With this in mind, how might we go about constructing right-chiral spinors from these same ingredients?
% %
% % The right-chiral field's Lagrangian must be subject to the same constraints as above, so it needs the same term cancelling $\partial_\nu S$ on the right.  And an additional term is needed to flip the sign of the intrinsic angular momentum -- this time with the gauge field multiplying from the left in place of the derivative.
% % \[ i\hat{\mathcal F}^\dag \varsigma^\mu \partial_\mu \hat{\mathcal F} + \hat{\mathcal F}^\dag \varsigma^\mu \hat{\mathcal F} \hat{\mathcal W_\mu} - n \hat{\mathcal F}^\dag \varsigma^\mu \hat{\mathcal W_\mu} \hat{\mathcal F} \]
% % where $n$ can be 0, 1, or 2 and still be consistent with angular momentum quantization.
% \[ i\hat{\mathcal F}^\dag S^\dag \varsigma^\mu (\partial_\mu S) \mathcal F + 2\hat{\mathcal F}^\dag S^\dag \varsigma^\mu (iS \partial_\mu S^\dag) S \mathcal F \]
% With the identity $S (\partial_\mu S^\dag) S = -\partial_\mu S$ for rotations, the effect of the new term is to flip the sign of angular momentum.

% For the sake of brevity, let us assume that the kinetic term for the components of $\mathcal W_\mu \equiv \mathcal W_\mu^a \varsigma^a$ is of the same form as that for the $SU(2)$ gauge field in the Standard Model, with the first order equivalent
% %
% % % \chapter{What is gauge invariance?}
% \begin{equation} \mathcal L = \Tr \left[ \mathcal G^{\mu\nu} \partial_\mu \mathcal W_\nu - i \mathcal G^{\mu\nu} \mathcal W_\nu \mathcal W_\mu - \tfrac14 \mathcal G^{\mu\nu} \mathcal G_{\mu\nu} \right] \end{equation}
% where the field strength $\mathcal G^{\mu\nu} \equiv \mathcal G^{\mu\nu}_a \varsigma^a$ transforms as $\Lambda^\mu_{\phantom\mu\mu'} \Lambda^\mu_{\phantom\mu\mu'} S \mathcal G^{\mu'\nu'} S^\dag$ under basis rotations.
% Subject to the first Lagrangian in \eqref{blah} (we denote this version as left-chiral), we are free to let the multivector field effectively transform as $\mathcal F \to S \mathcal F$, with $\mathcal W_\mu$ invariant and $\mathcal G^{\mu\nu} \to \Lambda^\mu_{\phantom\mu\mu'} \Lambda^\mu_{\phantom\mu\mu'} \mathcal G^{\mu'\nu'}$ under basis rotations.
% Furthermore, the left-chiral Lagrangian is invariant under a likewise unphysical transformation: $\mathcal F \to \mathcal F S^\dag$, $\mathcal W_\mu \to S \mathcal W_\mu S^\dag - i S \partial_\mu S^\dag$, $\mathcal G^{\mu\nu} \to S \mathcal G^{\mu\nu} S^\dag$.
% % For all intents and purposes, the latter \emph{is} a gauge transformation.

Since $\mathcal W_\mu$ occupies an edge position, it must be promoted to a field operator capable of mapping the quantum state to elements of the tangent space, and is in need of a kinetic term.
Let us assume that the kinetic term for the components of $\mathcal W_\mu \equiv \mathcal W_\mu^a \varsigma^a$ is of the same form as that for the $SU(2)$ gauge field in the Standard Model
, with the first order equivalent
\[ \mathcal L = \Tr \left[ \mathcal G^{\mu\nu} \partial_\mu \mathcal W_\nu - \tfrac18 \mathcal G^{\mu\nu} \mathcal G_{\mu\nu} \right] \]
If $\mathcal G^{\mu\nu}$ is anti-symmetric in its Greek indices, then the non-covariant term coming from the transformation of $\mathcal W_\nu$ -- which involves the second derivative of $S$ -- vanishes. But this Lagrangian has the same problem discussed above -- hanging outer transformation operators that cause problems when we promote fields to field operators.
\[ \mathcal L = \Tr \left[ \mathcal G^{\mu\nu} S^{-1} \partial_\mu (S \mathcal W_\nu) + S \mathcal G^{\mu\nu} S^{-1} \mathcal W_\nu \partial_\mu S^{-1} - \tfrac18 \mathcal G^{\mu\nu} \mathcal G_{\mu\nu} \right] \]
In order to construct a Lagrangian that can be transformed by inner linear operations alone, we can perform the same trick of adding a coupling term to $\mathcal W_\mu$
\[ \mathcal L = \Tr \left[ \mathcal G^{\mu\nu} \partial_\mu \mathcal W_\nu - i \mathcal G^{\mu\nu} \mathcal W_\nu \mathcal W_\mu \right] \]
This not only eliminates the outer transformation operators, but makes the kinetic Lagrangian invariant under basis transformations.
\[ \mathcal L = \Tr \left[ \mathcal G^{\mu\nu} S^{-1} \partial_\mu (S \mathcal W_\nu + i \partial_\nu S) - i \mathcal G^{\mu\nu} (\mathcal W_\nu + i S^{-1} \partial_\nu S) \mathcal W_\mu + \cdots \right] \]
The remaining new terms after the transformation are
\[ \delta \mathcal L = \Tr \left[ \mathcal G^{\mu\nu} (S^{-1} \partial_\mu S) \mathcal W_\nu + \mathcal G^{\mu\nu} ( S^{-1} \partial_\nu S) \mathcal W_\mu + \cdots \right] \]
which also vanish due to anti-symmetry of $\mathcal G^{\mu\nu}$.
\begin{equation} \mathcal L = \Tr \left[ \mathcal G^{\mu\nu} \partial_\mu \mathcal W_\nu - i \mathcal G^{\mu\nu} \mathcal W_\nu \mathcal W_\mu - \tfrac1{8} \mathcal G^{\mu\nu} \mathcal G_{\mu\nu} + \text{h.c.} \right] \end{equation}
% \begin{equation} \mathcal L = \Tr \left[ \mathcal G^{\mu} \partial_\mu \psi - i \mathcal G^{\mu\nu} \psi \mathcal W_\mu - \tfrac1{8} \mathcal G^{\mu} \mathcal G_{\mu} + \text{h.c.} \right] \end{equation}
% \begin{equation} \mathcal L = \Tr \left[ \mathcal G^{\mu} \partial_\mu (S \psi) - i \mathcal G^{\mu\nu} \psi \mathcal W_\mu - \tfrac1{8} \mathcal G^{\mu} \mathcal G_{\mu} + \text{h.c.} \right] \end{equation}
% where the field strength $\mathcal G^{\mu\nu} \equiv \mathcal G^{\mu\nu}_a \varsigma^a$ transforms as $\Lambda^\mu_{\phantom\mu\rho} \Lambda^\nu_{\phantom\nu\sigma} S \mathcal G^{\rho\sigma} \! S^\dag$ under basis rotations (or perhaps only as $S \mathcal G^{\mu\nu} \! S^\dag$, if the arguments in the opening miss the mark).
where each component of the field strength $\mathcal G^{\mu\nu}$ is a vector transforming with the basis.
Subject to the first Lagrangian in \eqref{blah} (we denote this version as left-chiral), we are free to let the multivector field effectively transform as $\mathcal F \to S \mathcal F$, with $\mathcal W_\mu$ invariant 
% and $\mathcal G^{\mu\nu} \to \Lambda^\mu_{\phantom\mu\mu'} \Lambda^\mu_{\phantom\mu\mu'} \mathcal G^{\mu'\nu'}$ 
under basis rotations.
Furthermore, the left-chiral Lagrangian is invariant under the likewise unphysical transformation \begin{equation} \mathcal F \to \mathcal F U^\dag , \quad \mathcal W_\mu \to U \mathcal W_\mu U^\dag - i U \partial_\mu U^\dag \label{gauge} \end{equation}
% , $\mathcal G^{\mu\nu} \to S \mathcal G^{\mu\nu} S^\dag$.
% For all intents and purposes, the latter \emph{is} a gauge transformation.
%
% If the second Lagrangian were to not result in any observable coupling between the physical degrees of freedom in the fields governed by its kinetic piece and $\mathcal W_\mu$, then one could be forgiven for concluding that the whole theory was invariant under that transformation.
%
%
where $U = \exp ( \frac i2 \alpha^j(\mathbf x) \varsigma^j )$, $\alpha^j \in \mathbb R$.  The second (right-chiral) theory in \eqref{blah} is not invariant under that transformation, unless its coupling to $\mathcal W_\mu$ -- which appears to vary with spin -- does not result in measurable effects.
% , which departs from the measured behavior of the weak gauge field.  
% If $\mathcal W_\mu$ is to be considered a physical field, then we must examine its kinetic term to determine which transitions are actually physical.
% If the kinetic term has the same form as that of the weak gauge field, 
% \[ \mathcal L_K = \Tr \, \mathcal G^{\mu}_{\phantom\mu\nu} \partial_\mu \mathcal W^\nu - i \mathcal G^{\mu}_{\phantom\mu\nu} \mathcal W^\nu \mathcal W_\mu - \tfrac14 \mathcal G^{\mu\nu} \mathcal G_{\mu\nu} \]

In the left-chiral theory, a transformation \eqref{gauge} can always align the degrees of freedom sourced by any state of $\mathcal F$ along one component $a$ of $\mathcal W^a_{\mu}$.  
If we had arrived at \eqref{blah} by elevating invariance under \eqref{gauge} to a principle, this would follow as a matter of course.  
But from our present vantage it can be appreciated as a great simplification, since for any single component $a$ of $\mathcal W^a_\mu$ there exist well behaved free plane wave solutions.
So an initial state with a left-chiral particle can evolve to a final state that includes a freely propagating excitation of $\mathcal W_\mu$.
% If we further assume that the global phase invariance of \eqref{foga} should be promoted to a local one in the usual manner involving an Abelian gauge field $B_\mu$, then we can pick out a basis coupling only to the combination $B_\mu + \mathcal W^3_\mu$.
% That one component can carry semiclassical plane wave solutions free of self-interactions on average.
In the right-chiral theory, on the other hand, all states of $\mathcal F$ couple to a mixture of Roman and Greek components of $\mathcal W^a_\mu$; classical solutions must account for self-interaction among the various Roman components.  Semi-classical momenta-conserving transitions producing long- or even relatively short-range interactions with effects accessible to experiment may as a result be prohibited or constrained in interesting ways.
% , insulating the right-chiral field from interaction with the weak sector.
% , whereas only states that excite just one Roman component $\mathcal G_a^{\mu\nu}$ can participate in a semi-classical momenta-conserving transition.
% (The self-interacting system $\{\mathcal G^{\mu\nu}_a,\mathcal W_\lambda^b \}$ has no classical plane wave solutions for which a gauge transformation cannot align all of the oscillating degrees of freedom along one component $a$ of $\mathcal G_a^{\mu\nu}$.)
% Starting from the first order formulation of electromagnetism and using the same 
% \[ \mathcal L_K = \Tr \, \mathcal G^{\mu}_{\phantom\mu\nu} \partial_\mu \mathcal W^\nu - i G^{\mu}_{\phantom\mu\nu} \mathcal W^\nu \mathcal W_\mu - \tfrac14 \mathcal G^{\mu\nu} \mathcal G_{\mu\nu} \]
An investigation into the transitions allowed in the right-chiral theory would be of value.

A loose end concerns the basis transformation under boosts, in which the kinetic term becomes
$ \Tr {[i S^{-2} \mathcal F S^\dag \varsigma^\mu S \partial_\mu \mathcal F]} $.
($\mathcal W_\mu$ must also transform under boosts, but the resulting non-covariant additive term is left out when we take the Hermitian part.)
Consistency and overall Lorentz invariance suggest that we should introduce another auxiliary field transforming as a four-vector with the tangent basis, $\varepsilon \equiv \varepsilon^\mu \varsigma_\mu \to S \varepsilon S^\dag$, to occupy the left-most position and absorb stray factors of $S^{-1}$.
% Alternatively, we can loosen the requirement that all outer transformation operators can be omitted to only matter for consistent basis and coordinate transformations acted together.
Alternatively, since no derivatives of $S$ end up in the Lagrangian for boosts, we could try to rig the particle annihilation and creation operators to transform in a compensatory way.  But even if such a trick worked mathematically, we suspect it would be difficult to justify in the same spirit as the arguments motivating this work.
% \[ \mathcal L = i \varepsilon \psi^\dag \varsigma^\mu \partial_\mu \psi + \varepsilon \psi^\dag \varsigma^\mu \psi \mathcal W_\mu + \cdots \]

With the elephant in the room now properly named, we substitute $\{\sigma^i,\psi\} \in SL(2,\mathbb C)$ for $\{\varsigma^i,\mathcal F\}$ to yield a provisional final form
\begin{equation}
\mathcal L = i\varepsilon\psi^\dag \sigma^\mu \partial_\mu \psi + \begin{cases} \varepsilon \psi^\dag \sigma^\mu \psi \mathcal W_\mu + i \varepsilon \psi^\dag \sigma^\mu \omega_\mu \psi & \text{(L)} \\
 \varepsilon \psi^\dag \sigma^\mu \psi \mathcal W_\mu - 2 \varepsilon \psi^\dag \sigma^\mu \mathcal W_\mu \psi - i \varepsilon \psi^\dag \sigma^\mu \omega_\mu \psi & \text{(R)}
 \end{cases}
 \label{final}
\end{equation}
% When $\textstyle \varepsilon^\mu = (\, 1 \, 0 \, 0 \, 0 \,)$, the time-like component $\varepsilon^0$ couples to $\mathcal L$ from \eqref{final}.   if $\psi_{\text{L}}$ and $\psi_{\text{R}}$ acquire mass via a term not tracked by $\varepsilon^\mu$, then $\varepsilon^0$ would couple to that mass in the classical limit.  
%
Since $\mathcal F$/$\psi$ are algebraic elements rather than column vectors, the representation we adopt for the geometric algebra makes no significant difference.
% But it does not hurt to use the more familiar representation of the Pauli matrices.)  
In the corresponding quantum theory, all of the fields occupying outer positions, including $\varepsilon$, must correspond to field operators with kinetic terms.  
The principle invoked here has nothing to say on the statuses of the spin connection $\omega_\mu$ and the hitherto suppressed metric $g_{\mu\nu}$ or tetrads $e^{a}_{\phantom a \mu}$ as field operators versus mere bookkeeping devices without representation in the state space.

% If we only require that under consistent basis \emph{and} coordinate transformations, then $\varepsilon$ could transform with the coordinates.

In summary, a misguided attempt to write down a first order Lagrangian for the Faraday tensor, followed by some minimal corrective measures respecting the ethos of geometric algebra, yields a proto-theory containing left- and right-chiral effective spin-$\tfrac12$ fields.  In that framework, all of the underlying geometric objects are left invariant by a homogeneous rotation by $2\pi$ radians, and the two chiralities couple differently to a gauge-like field in a manner that is intimately tied to their geometric character.  

==> Trash/inflation_background.tex <==
\section{Cosmology Before 1980}
    Briefly discuss the development of cosmology from speculation to science with the predictions of general relativity and the advent of technologies for collecting observational data, the cosmic microwave background, etc.
    
    \subsection{Friedmann-Lama\^itre-Robertson-Walker Spacetime}
        If science had Fundamental Theorems, that of cosmology would be that the universe is approximately homogeneous and isotropic when considered at sufficiently large scales.
        This principle is borne out by observation.
        
        The Friedmann-Lema\^itre-Robertson-Walker (FLRW) metric describes a spacetime that is homogeneous and isotropic, possessing maximal symmetry on a preferred family of space-like hypersurfaces.  The line element takes the form
        \begin{equation} \dx s^2 = -\dx t^2 + a(t)^2 \left( \frac{\dx r^2}{1-k r^2} + r^2 \,\dx\Omega_2 \right) \label{flrw} \end{equation}
        \begin{equation} \dx s^2 = a(\tau)^2 \left( -\dx \tau^2 +  \frac{\dx r^2}{1-k r^2} + r^2 \,\dx\Omega_2 \right) \label{flrw_conformal} \end{equation}
        where $a(t)$ is the \emph{scale factor}, $k$ specifies the Gaussian curvature on hypersurfaces of constant $t$, and $\dx\Omega_2 \equiv \dx\theta^2 + \sin^2 \theta \, \dx\phi^2$ is the solid angle element on the 2-sphere.
        Special cases include the maximally symmetric (time included) de Sitter and anti-de Sitter space, for which the scale factor takes the form $a(t) = \exp{(\pm Ht)}$  From the scale factor, we may define the Hubble parameter
        \[ H \equiv \frac{\dot a}{a} \]
        
        When sourced by a perfect fluid (e.g. a non-interacting dust) with uniform density $\rho$ and pressure $p$, the Einstein field equations yield the Friedmann equations.
        \begin{equation} H^2 = \frac{8\pi G}{3} \rho - \frac{k}{a^2} \label{friedmann1} \end{equation}
        \begin{equation} \dot H + H^2 = -\frac{4\pi G}{3} \rho (1 + 3w) \label{friedmann2} \end{equation}
    \subsection{Naturalness Problems in the Big Bang Picture}
    
    Three problems related to the perceived naturalness of the Big Bang picture drove model development in the 1970s and 80s.
    
    The horizon problem relates to how distant regions of space that could never be in thermal contact according to the Big Bang picture nonetheless appear to have come to thermal equilibrium.
    The temperature variation deduced from anisotropy data from the CMB is one part in $10^5$.
    
    The flatness problem concerns why the spatial curvature on hypersurfaces appears to be very close to flat, when Einstein's equation sourced by matter and radiation in the abundances used the Big Bang model predict that the spatial curvature $k$ should quickly depart from zero given any initial deviation.
    
    The monopole problem addresses the fact that we do not detect magnetic monopoles, though Grand Unified Theories under serious study at the time predicted their production in large quantities at energy scales signaling Grand Unification.
    
\section{Inflation}
In response to the problems discussed above -- primarily the problem of the apparent scarcity of gauge monopoles -- Guth proposed a new cosmological model in which the Universe goes through a sustained epoch resembling de Sitter space.
In this model, a scalar field $\phi$ acquires an expectation value corresponding to a positive energy density derived at a false vacuum of its potential $V(\phi)$.
\[ \mathcal L = \tfrac12 \partial_\mu \phi \partial^\mu \phi - V(\phi) \]

    \subsection{Old Inflation and its Problems}
    before undergoing a phase transition to much different behavior.
    
    In Guth's original model, a scalar field $\phi(t)$, assumed isotropic, with potential energy density $V(\phi)$ is responsible for sourcing Einstein's field equations as an effective perfect fluid, with energy density and isotropic pressure
    \[ \rho = \tfrac 12 \dot\phi^2 + V(\phi) \qquad p = \tfrac12 \dot\phi^2 - V(\phi) \]
    The scalar field was to be subject to a potential function $V(\phi)$ with one or more meta-stable false minima, in which the scalar field becomes trapped for a time, with $\dot\phi \ll \sqrt{2 V(\phi)}$.
    In this configuration, the equation of state takes the form $w(p) = -\rho$, and the Friedmann equations dictate an exponential form for the scale factor defined with respect to flat space-like hypersurfaces ($k=0$) -- effectively evolving as de Sitter space. 
    Treating the potential barrier quantum mechanically, there is some probability for bubbles to nucleate into a neighboring basin containing the true minimum, where ordinary cosmic evolution may resume.
    
    This original model of inflation did not work because the nucleation rate was too slow to produce large thermalized regions that preserve the desired homogeneity and isotropy of the background after inflation.
    After the bubble nucleates, pressure on the inside is greater than outside the bubble wall, causing the membrane to quickly accelerate to near the speed of light.  But meanwhile, the background space continues to inflate, and only bubbles that nucleate in very close proximity have a chance of merging.
    \subsection{New Inflation}
% \chapter{Quantum Theory of the Inflaton}
From its beginning in Old Inflation, the framework has relied on quantum effects, taking its place in a new era of quantum cosmology.  With observations of Cosmic Microwave Background revealing difficult-to-explain inhomogeneities, and the implication from inflation that distance scales the size of our Observable Universe were once on the order of the atomic scales were quantum effects come into play, a need arose for precise predictions accounting for quantum behavior of the scalar field sourcing inflationary expansion.

For a homogeneous scalar field $\phi(t)$, the equation of motion coupled to the curved background spacetime characterized by $H \equiv \dot a/a$ is
\begin{equation} \nabla_0 (\partial_0\phi) = \ddot \phi + 3 H \dot\phi = -\ddx{V}{\phi} \label{eomphihomogeneous} \end{equation}
The field need not be time-indepdent to ensure a nearly constant Hubble parameter; rather, we need only that
\begin{equation} \frac12 \dot\phi^2 \ll V(\phi) \qquad \ddot\phi \ll V_{,\phi} \label{slowrollconditions_raw} \end{equation}
\[ \dot\rho = -3 H (\rho + p) \]
% These are the {\it slow roll} conditions
% under which the speed $\dot\phi$ and the Hubble parameter remain nearly constant. 
The first of these {\it slow roll} conditions ensures that the equation of state for $\phi$ takes the form $p \approx -\rho$, the same as that for dark energy.  As a result, the Friedmann equations become a requirement that the Hubble parameter is nearly constant in time: $\dot H = 0$.
The second ensures that $\dot\phi$ does not grow quickly so as to render the first invalid; in that approximation, the equation of motion for $\phi$ becomes
\begin{equation} 3 H \dot\phi = -V_{,\phi} \label{eomslowroll} \end{equation}

Inflation ends when the slow roll conditions are strongly broken; most of the field's potential energy is converted into kinetic energy, and the rapidly varying inflaton deposits energy into quanta of other fields to which it is coupled, contributing to matter and radiation equations of state.

\section{Evidence for the Inflationary Picture}
    \paragraph{Parametrization of Perturbation Spectrum}
    \[ P_s(k) = A_s \left( \frac{k}{k^\star} \right)^{1-n_s+\alpha_s \ln k + \cdots} \]
\section{Viability of Existing Models}
    % \subsection{Simplest Models}
    % \subsection{Single and Multifield}
    % \subsection{Higgs Inflation}
    % \subsection{Hybrid Inflation}
    % \subsection{Slow Roll Attractor}

==> conclusion.tex <==
Inflation has been demonstrated to be highly successful as a paradigm for early universe cosmology, addressing naturalness problems lingering in the Big Bang picture while offering a coherent explanation for the origin of primordial curvature  perturbations implied by observations of the  Cosmic Microwave Background.
%
Its grandest prediction of all may be that we live in an eternally inflating multiverse, producing an unbounded number of causally disconnected regions with wildly varying cosmological histories.

% \paragraph{What We Did}
%
For research culminating in this dissertation, we investigated whether and to what extent eternality can or must be considered a genuine prediction of inflation -- in the sense of following generically from conditions giving rise to the latter in the context of more-or-less physically-justifiable measures on the space of inflationary cosmologies.
We shed light on how one would go about evaluating claims that features of a model are generic or fine-tuned.
%We extended the work of Tegmark to explore the implications of adopting various simple measures over the space of inflation models and initial conditions, on the likelihood of eternal inflation in its three broad instantiations.
Using a computational methodology developed to assess the typicality of eternal inflation with applied statistics,
we found that genericity is highly dependent on the measure, and that its determination inevitably involves some nuance.
%Measures in which the field is initialized near the top of the barrier are generically eternal by the topological mode, while stochastic eternal inflation may not be generic at sub-Plancking field scales.
%Uniform sampling of the 
%
In Appendix A, we go on to explore the toy landscape of Gaussian random potential functions in conjunction with computable measures over initial conditions, probing characteristics of eternal inflation like the fractal dimension.
We demonstrate the absence of an informative relationship between the running of the spectral index and presence of stochastic eternal inflation in models with a uniform sampling of initial field values.
% (For these results, see Appendix~\ref{pt:explorations}.)

%\paragraph{What is the Impact?}
This work adds to an ongoing conversation pertaining to the credibility of the anthropic view of the cosmos that has gained traction in recent decades.
Whether or not eternal proliferation and a ``multiverse'' generically follow from inflation has profound implications for this picture, as anthropic arguments require a large population of trial sites where apparently fine-tuned quantities can vary.
%
In addition to direct scholarly contribution, we intend to publish a code package for simulating inflation across an ensemble of randomly generated inflaton potentials using modern programming tools; others may build upon this package in furtherance of related research objectives.


% \paragraph{Is Naturalness Real?}
There may be no way of assigning probabilities to partitions of the space of cosmological models that is not contaminated by human prejudice.
If that were the case, should any weight be assigned to the intuitions and conceptual biases of scientists and philosophers in judging the credibility of proposals that elude falsification by evidence?  Or should we be content with remaining agnostic when apparent naturalness problems crop up in our scientific theories?

The answer to this question depends largely on the dispositon of the answerer with respect to the role of science.
If the objective in science is limited to illucidating the reproducible, experimental facts of the natural world, then the scientist should pay little attention to naturalness problems, which by their nature evade unambiguous framing and definitive closure (except perhaps by the supersession of the paradigm that is the context for the problem).
If, on the other hand, one views science as in some respects a form of elite art -- to be appreciated in detail by a highly trained community of experts and in likeness by the general public -- then aesthetic and philosophical questions are fair game, and perhaps the whole point of the enterprise.
